TRAIL: Towards Effective Log Parsing for Rare Logs through Template-Preserving Augmentation

Log parsing is essential for system log analysis because it supports tasks such as debugging, monitoring, and anomaly detection by transforming unstructured log messages into structured log templates. However, real-world log datasets exhibit highly imbalanced, long-tailed distributions, where a small number of frequent templates dominate while many rare templates appear only a few times. This imbalance causes evaluation results to be overly optimistic by allowing frequent templates to dominate benchmark metrics, while poor performance on rare yet operationally important events remains largely hidden. In this paper, we investigate the prevalence and impact of rare log groups, defined as log groups with fewer than five instances. Our empirical study on the widely used Loghub-2.0 benchmark shows that rare log groups account for nearly 20% of all templates but less than 0.01% of log messages. Because they contain only a handful of instances, all evaluated parsers experience substantial performance degradation on these groups. To address this challenge, we propose TAILOR, a log parsing framework that improves template inference for rare log groups through template-preserving augmentation. TAILOR enriches rare log groups with template- consistent log messages before template inference. The additional structural evidence helps distinguish static tokens from dynamic variables. Our experimental results show that TAILOR improves parsing accuracy on rare log groups by 19% over the strongest baseline while maintaining competitive performance on complete datasets. We further show that the proposed augmentation strategy generalizes across different LLM backbones and consistently improves existing LLM-based parsers without modifying their core architectures.

==> figures/Boxplot.tex <==
\begin{figure*}[H]
    \centering
    \includegraphics[width=\linewidth,height=2cm, keepaspectratio]{figures/Box_plot.png}
    \caption{Robustness comparison between baselines and SEPLOG on entire datasets}
    \label{fig:boxplot}
\end{figure*}

==> figures/GeneralizeTable.tex <==
\begin{table*}[t]
\centering
\caption{Performance comparison across datasets and LLMs using PA, GA, FTA, and FGA.}
\label{tab:generalize}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|l|ccccccccccccc}
\toprule
\multicolumn{3}{c|}{\textbf{Datasets}} 
& Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac & OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper \\
\midrule

\multirow{8}{*}{\textbf{Llama}} 
& \multirow{4}{*}{\textbf{SEPLOG}} 
& PA  & 0.50 & 0.60 & 0.57 & 1.00 & 0.96 & 0.65 & 0.57 & 0.51 & 0.89 & 0.66 & 0.46 & 0.43 & 0.66 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.92 & 0.95 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\
& & FTA & 0.50 & 0.60 & 0.50 & 1.00 & 0.92 & 0.64 & 0.59 & 0.41 & 0.75 & 0.66 & 0.47 & 0.44 & 0.71 \\
& & FGA & 1.00 & 0.90 & 1.00 & 1.00 & 1.00 & 1.00 & 0.90 & 0.96 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\

& \multirow{4}{*}{\textbf{LibreLog}} 
& PA  & 0.50 & 0.30 & 0.46 & 0.40 & 0.55 & 0.46 & 0.35 & 0.23 & 0.22 & 0.66 & 0.14 & 0.35 & 0.33 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.96 & 0.97 & 1.00 & 1.00 & 1.00 & 0.98 & 1.00 \\
& & FTA & 0.50 & 0.30 & 0.44 & 0.75 & 0.53 & 0.50 & 0.51 & 0.32 & 0.57 & 0.66 & 0.43 & 0.33 & 0.71 \\
& & FGA & 1.00 & 0.30 & 0.11 & 0.00 & 0.15 & 0.28 & 0.07 & 0.15 & 1.00 & 0.12 & 0.30 & 0.13 & 0.14 \\
\midrule

\multirow{8}{*}{\textbf{Gemma}} 
& \multirow{4}{*}{\textbf{SEPLOG}} 
& PA  & 0.50 & 0.30 & 0.256 & 1.00 & 0.44 & 0.07 & 0.28 & 0.11 & 0.39 & 0.23 & 0.05 & 0.17 & 0.33 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 0.63 & 1.00 & 0.97 & 0.83 & 1.00 & 0.81 & 1.00 & 0.89 & 1.00 \\
& & FTA & 0.50 & 0.30 & 0.195 & 1.00 & 0.428 & 0.14 & 0.23 & 0.10 & 0.25 & 0.20 & 0.09 & 0.18 & 0.42 \\
& & FGA & 1.00 & 0.90 & 1.00 & 1.00 & 0.66 & 1.00 & 0.97 & 0.84 & 1.00 & 0.34 & 1.00 & 0.88 & 1.00 \\

& \multirow{4}{*}{\textbf{LibreLog}} 
& PA  & 0.50 & 0.20 & 0.24 & 0.00 & 0.44 & 0.07 & 0.22 & 0.10 & 0.16 & 0.00 & 0.02 & 0.16 & 0.33 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.98 & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 \\
& & FTA & 0.50 & 0.30 & 0.17 & 0.00 & 0.13 & 0.14 & 0.18 & 0.09 & 0.12 & 0.00 & 0.04 & 0.16 & 0.42 \\
& & FGA & 1.00 & 0.30 & 0.08 & 0.00 & 0.14 & 0.28 & 0.07 & 0.11 & 0.12 & 0.00 & 0.30 & 0.13 & 0.14 \\
\midrule

\multirow{8}{*}{\textbf{Mistral}} 
& \multirow{4}{*}{\textbf{SEPLOG}} 
& PA  & 0.50 & 0.60 & 0.46 & 1.00 & 0.74 & 0.61 & 0.60 & 0.40 & 0.67 & 0.33 & 0.36 & 0.45 & 0.56 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 & 0.96 & 1.00 & 1.00 & 1.00 & 0.96 & 1.00 \\
& & FTA & 0.50 & 0.70 & 0.41 & 1.00 & 0.56 & 0.57 & 0.60 & 0.35 & 0.62 & 0.33 & 0.39 & 0.45 & 0.57 \\
& & FGA & 1.00 & 0.90 & 1.00 & 1.00 & 0.83 & 1.00 & 0.97 & 0.95 & 1.00 & 1.00 & 1.00 & 0.93 & 1.00 \\

& \multirow{4}{*}{\textbf{LibreLog}} 
& PA  & 0.00 & 0.40 & 0.38 & 0.40 & 0.51 & 0.42 & 0.40 & 0.35 & 0.38 & 0.33 & 0.09 & 0.37 & 0.55 \\
& & GA  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.97 & 1.00 & 1.00 & 1.00 & 0.97 & 1.00 \\
& & FTA & 0.00 & 0.50 & 0.38 & 0.50 & 0.46 & 0.35 & 0.35 & 0.32 & 0.25 & 0.33 & 0.17 & 0.34 & 0.57 \\
& & FGA & 1.00 & 0.30 & 0.11 & 0.00 & 0.15 & 0.28 & 0.07 & 0.16 & 0.12 & 1.00 & 0.30 & 0.13 & 0.14 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/Table0.tex <==
% No extra packages required

\begin{table}[tb]
  \centering
  \caption{Dataset distribution and rarity statistics}
  \label{tab:Table0}

  % Tighten spacing a bit (both are core LaTeX)
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.05}

  % 10 columns total. Fixed widths so it fits \columnwidth.
  % 0.20 + 9*0.086 = 0.974 of \linewidth (safe margin)
  \begin{tabular}{ p{0.13\linewidth}
                   |p{0.088\linewidth} p{0.086\linewidth}
                   p{0.088\linewidth} p{0.086\linewidth} p{0.086\linewidth}
                   p{0.088\linewidth} p{0.086\linewidth} p{0.086\linewidth} }
    \hline
    \textbf{Dataset} &
    \shortstack{\textbf{\# Total}\\\textbf{Logs}} &
    
    \shortstack{\textbf{\% in}\\\textbf{Top10}} &
    \shortstack{\textbf{\# Groups}\\\textbf{with 50\%}} &
    \shortstack{\textbf{Total \#}\\\textbf{Groups}} &
    \shortstack{\textbf{\# Groups}\\\textbf{$<$5}} &
    \shortstack{\textbf{Total \#}\\\textbf{Rare Logs}} &
    \shortstack{\textbf{\% Rare}\\\textbf{Logs}} &
    \shortstack{\textbf{\% Groups}\\\textbf{$<$5}} \\
    \hline
    MAC         & 100,315          & 26\% & 40  & 626  & 175 & 331 & 0.03\%    & 27\% \\
    HealthApp   & 212,395          & 87\% & 5   & 156  & 12  & 27  & 0.001\%   & 7\%  \\
    HPC         & 429,989          & 83\% & 5   & 74   & 13  & 26  & 0.00006\% & 17\% \\
    Thunderbird & 16,601,746       & 53\% & 10  & 1,242& 316 & 682 & 0.004\%   & 25\% \\
    OpenStack   & 207,633          & 71\% & 3   & 49   & 3   & 6   & 0.00002\% & 6\%  \\
    Apache      & 51,979          & 98\% & 3   & 29   & 2   & 3   & 0.0003\%  & 7\%  \\
    BGL         & 4,631,262       & 76\% & 3   & 320  & 26  & 53  & ~0  & 8\%  \\
    Linux       & 23,922          & 82\% & 3   & 338  & 65  & 154 & ~0  & 19\% \\
    OpenSSH     & 638,948         & 92\% & 3   & 38   & 6   & 15  & ~0  & 15\% \\
    Hadoop      & 179,994         & 59\% & 6   & 236  & 35  & 78  & ~ 0  & 14\% \\
    Zookeeper   & 74,274          & 83\% & 4   & 89   & 7   & 18  & ~0  & 12.7\% \\
    HDFS        & 11,167,741      & 99\% & 3   & 40   & 8   & 7   & ~0  & 8\%  \\
    Spark       & 16,075,118      & 87\% & 4.5 & 236  & 23  & 41  & ~0  & 9\%  \\
    Proxifier   & 21,321          & 99\% & 1   & 11   & 0   & 0    & ~0 & 0\%  \\
    \hline
  \end{tabular}
\end{table}


==> figures/Table1.tex <==
\begin{table}[tb]
  \centering
  \caption{Example of LibreLog parsing  accuracy on frequent vs infrequent log events}
  \label{tab:Table1}
  \scriptsize
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.05}
  \begin{tabular}{l|rrrp{0.56\columnwidth}} % <-- wrap last column
    \toprule
    \textbf{EventId} & \textbf{Number of logs} & \textbf{Data ratio} & \textbf{LibreLog\_PA} & \textbf{Template Expected} \\
    \midrule
    E213 & 40126 & 40.0\% & 100\% & Cocoa scripting error for \texttt{<*>}: four character codes must be four characters long. \\
    E164 & 1 & < 0.1\% & 0\% & \texttt{handle\_will\_sleep\_auth\_and\_shield\_windows}: Ordering out authw \texttt{<*>} (\texttt{<*>}), shield \texttt{<*>} (\texttt{<*>}) (lock state: \texttt{<*>}). \\
    \bottomrule
  \end{tabular}
\end{table}


==> figures/Table2.tex <==
\begin{table}[tb]
\centering
\caption{Parsing accuracy of LibreLog on frequent vs.\ infrequent logs}
\label{tab:Table2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|llllllll} % <-- vertical line only after Dataset
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c}{\textbf{Frequent logs}} & \multicolumn{4}{c}{\textbf{Infrequent logs}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& PA & GA & FTA & FGA & PA (\% \gain{↑}/\drop{↓}) & GA (\% \gain{↑}/\drop{↓}) & FTA (\% \gain{↑}/\drop{↓}) & FGA (\% \gain{↑}/\drop{↓}) \\
\midrule
Apache & 0.98 & 0.98 &0.78&0.76& 0.50 (48\% \drop{↓}) & 0.50(1\%\gain{↑})&0.50(2\% \drop{↓})&1(23\% \gain{↑})\\
BGL       &0.95 & 0.90 & 0.71&0.64&0.41 (57\%\drop{↓}) & 0.96 (5\%\gain{↑})&0.40(2\% \drop{↓})&0.94(23\% \gain{↑})\\
Hadoop        & 0.74 & 0.93 &0.71&0.66&0.60 (19\%\drop{↓}) & 1.00 (8\%\gain{↑})&0.58(-)&1(39\% \gain{↑}) \\
HDFS         & 0.97 & 0.93 & 0.95&0.87&0.80 (17\%\drop{↓}) & 1 (14\% \gain{↑})&0.75(9\% \drop{↓})&1(13\% \gain{↑})\\
HealthApp      & 0.94 & 0.85 &0.74&0.69&0.88 (6\% \drop{↓}) & 1 (16\%\gain{↑})&0.75(17\% \gain{↑})&1(36\% \gain{↑})\\
HPC     & 0.92 & 0.73 &0.62&0.61&0.65 (29\%\drop{↓}) & 1 (26\% \gain{↑})&0.42(4\% \drop{↓})&1(14\% \drop{↓})\\
Linux      & 0.75 & 0.80 & 0.49&0.48&0.70 (6\% \drop{↓}) & 0.90 (11\% \gain{↑})&0.67(6\% \gain{↑})&0.89(60\% \gain{↑})\\
Mac   & 0.66&0.85 &0.44&0.34&0.48 (48\%\drop{↓})&0.90 (4\% \gain{↑})&0.43(-)&0.92(129\% \gain{↑})\\
OpenSSH       & 0.26&0.60 &0.53&0.44&0.44 (69\%\gain{↑}) &0.61 (-)&0.51(1\% \gain{↑})&0.80(54\%\gain{↑})\\
OpenStack   & 0.76&0.76 &0.76 &0.50&0.66 (13\%\drop{↓})&1 (29\% \gain{↑})&0.66(2\% \gain{↑})&1(6\%\gain{↑})\\
Spark     &0.88 & 0.87&0.69&0.66&0.46 (47\%\drop{↓}) &0.90 (2\% \gain{↑})&0.45(2\% \drop{↓})&0.93(33\% \drop{↓})\\
Thunderbird   & 0.63&0.72 &0.41&0.45&0.53 (15\%\drop{↓}) &0.86 (17\%\gain{↑})&0.48(20\% \gain{↑})&0.90(84\% \gain{↑})\\
Zookeeper  & 0.84&0.98 &0.85&0.75&0.66 (21\%\drop{↓}) &1 (33\%\drop{↓})&0.71(1\% \drop{↓})&1(30\% \gain{↑})\\
%Proxifier   &0.51 & 0.89&- &-\\
\midrule
Average &0.81 &0.82 &0.72&0.57&0.54(33\%\drop{↓})&0.89(8\%\gain{↑})&0.48(33\%\drop{↓})&0.87(52\%\gain{↑})\\
\bottomrule
\end{tabular}%
}
\end{table}


==> figures/Table2_0_.tex <==
\begin{table*}[t]
  \centering
  \caption{Parsing accuracy of LibreLog on frequent vs.\ infrequent logs}
  \label{tab:Table2}
  \scriptsize
  \setlength{\tabcolsep}{10pt} % tighten column separation
  \renewcommand{\arraystretch}{1.5} % slightly tighter rows

  \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} &
      \multicolumn{2}{c}{\textbf{Frequent logs}} &
      \multicolumn{2}{c}{\textbf{Infrequent logs}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & PA & GA & PA (\% \gain{↑}/\drop{↓}) & GA (\% \gain{↑}/\drop{↓}) \\
    \midrule
Mac         & 0.65 & 0.81 & 0.23 (46\% \drop{↓}) & 0.95 (16\% \gain{↑}) \\
Thunderbird & 0.69 & 0.86 & 0.35 (49\% \drop{↓}) & 0.98(13\%\gain{↑})\\
Linux       &0.69 & 0.86 & 0.35 (66\%\drop{↓}) & 0.96 (5\%\gain{↑})\\
HPC         & 0.92 & 0.90 & 0.46 (50\%\drop{↓}) & 1.00 (16\%\gain{↑}) \\
BGL         & 0.90 & 0.90 & 0.33 (63\%\drop{↓}) & 0.96 (6\% \gain{↑})\\
Spark       & 0.88 & 0.85 & 0.14 (84\% \drop{↓}) & 1.00 (15\%\gain{↑})\\
OpenSSH     & 0.49 & 0.86 & 0.22 (55\%\drop{↓}) & 1.00 (14\% \gain{↑})\\
Hadoop      & 0.87 & 0.96 & 0.46 (47\% \drop{↓}) & 1.00 (4\% \gain{↑})\\
Zookeeper   & 0.99&0.84 &0.33 (60\%\drop{↓})&1.00 (1\% \gain{↑})\\
HDFS        & 1.00&1.00 &0.0.4 (6\%\drop{↓}) &1.00 (-)\\
HealthApp   & 0.86&0.97 & 0.55 (36\%\drop{↓})&1.00 (20\% \gain{↑})\\
Apache      &1.00 & 0.99&0.5 (5\%\drop{↓}) &1.00 (-)\\
OpenStack   & 0.81&0.83 &0.66 (18\%\drop{↓}) &1.00 (19\%\gain{↑})\\
    \midrule
    Average     & 0.83 & 0.89 & 0.50                 & 0.92                  \\
    \bottomrule
  \end{tabular}
\end{table*}

==> figures/Table3.tex <==
\begin{table}[tb]
  \centering
  \caption{SEPLOG Parsing and Grouping accuracy comparison focusing on rare logs with state-of-the-art (Librelog). \anran{into a barchart --> see example\_barchart.png under the figures folder}}
  \label{tab:Table3}
  \small
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.0}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l|cccccc}
    \toprule
    \textbf{Dataset} & \textbf{\#rare logs} & \textbf{LIBRELOG\_PA} & \textbf{LIBRELOG\_GA} & \textbf{SEPLOG\_PA} & \textbf{SEPLOG\_GA} \\
    \midrule
    Mac          & 331 & 0.35 & 0.97 & 0.57 & 0.97 \\
    Linux        & 154 & 0.54 & 0.96 & 0.66 & 0.97 \\
    HPC          & 26  & 0.57 & 1.00 & 0.66 & 1.00 \\
    Hadoop       & 78  & 0.58 & 1.00 & 0.576 & 1.00 \\
    BGL          & 53  & 0.48 & 0.96 & 0.58 & 1.00 \\
    HDFS         & 10  & 0.80 & 1.00 & 0.80 & 1.00 \\
    OpenSSH      & 15  & 0.44 & 1.00 & 0.50 & 1.00 \\
    Spark        & 41  & 0.41 & 1.00 & 0.41 & 1.00 \\
    Thunderbird  & 682 & 0.43 & 0.98 & 0.53 & 0.96 \\
    Zookeeper    & 18  &0.60  & 1 & 0.7 &1  \\
    HDFS         & 10  & 0.33 & 1 & 1 & 1 \\
    HealthApp    & 27  & 0.69 & 1 & 0.96 & 1 \\
    Apache       &  2 & 0.5 & 1 & 0.5 & 1 \\
    OpenStack    &  6 & 0.66 & 1 & 0.66 & 1 \\
    \bottomrule
    %\midrule
    Average &0.52 & 0.98&0.60&0.99\\
\bottomrule
  \end{tabular}}
\end{table}


==> figures/Table4.tex <==
\begin{table}[t]
  \centering
  \caption{Improvement in PA after augmentation for rare event logs}
  \label{tab:Table4}
  \small
  \setlength{\tabcolsep}{8pt}
  \renewcommand{\arraystretch}{1.5}
  \begin{tabular}{l|cc}
    \hline
    \textbf{EventId} & \textbf{PA before augmentation} & \textbf{PA after augmentation} \\
    \hline
    E164 (Mac) & 0\% & 100\% \\
    \hline
  \end{tabular}
\end{table}


==> figures/TableResult.tex <==
\begin{table}[tb]
\centering
\caption{SEPLOG parsing and grouping accuracy (PA, GA) and template-level metrics (FTA, FGA) compared with state-of-the-art methods.}
\label{tab:Table5}
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} 
& \multicolumn{4}{c|}{\textbf{SEPLOG}} 
& \multicolumn{4}{c|}{\textbf{LibreLog}} 
& \multicolumn{4}{c}{\textbf{Drain}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA \\
\midrule
%
%Apache      & 0& 0 &1  &1  & 0.5 &0.5  &1  &1  &0.5  &0.5  &1  &1   \\
%BGL         & 0.13 &0.19  &0.96  & 0.94 & 0.33 &0.34  &0.96  &0.30  &0.57  &0.61  &0.94  &0.94  \\
%Hadoop      & 0.29 &0.19  &1  &1  & 0.46 & 0.44 & 1 & 0.11& 0.57 & 0.50 &1  &1  \\
%HDFS        & 0 & 0 & 1 &  &0.4  &0.75  &1  &0  &1  &1  &1  &1    \\
%HealthApp   & 0.48 &0.3  &1  &1  &0.55  &0.53  &1  &0.15  &0.96  &0.92  &1  &1  \\
%HPC         & 0.038 &0.07  &1  &1  & 0.46 & 0.5 &1  &0.28  & 0.65 & 0.64 &1  &1  \\
%Linux       & 0.29 &0.28  &0.90  &0.95  &0.35  & 0.51 & 0.96 &0.065  &0.57  &0.59  &0.92  &0.90  \\
%Mac         & 0.13 &0.14  &0.91  &0.93  &0.23  &0.32  &0.97  &0.15  &0.51  &0.41  & 0.95 & 0.957\\
%OpenSSH     &  0.27& 0.37 & 1 & 1 & 0.22 & 0.57 & 1 & 1 & 0.89 & 0.75 & 1 & 1 \\
%OpenStack   & 0.33 & 0.33 & 1 &1  & 0.66 & 0.66 &1  &0.12  &0.66  &0.66  & 1 & 1 \\
%Spark       & 0.17 & 0.17 & 1 & 1 &0.14  & 0.43 & 1 & 0.30 &0.46  &0.47  &1  &1  \\
%Thunderbird & 0.17 & 0.18 &0.95  &0.94  &0.35  & 0.33 & 0.98 & 0.13 & 0.43 & 0.44 &0.95  &0.95  \\
%Zookeeper   & 0.44 & 0.57 & 1 & 1 & 0.33 &0.71  & 0.1 & 0.14 & 0.66 & 0.71 &1  &1  \\
%

Apache      	&0.5&	1&	0.5&	1&	0.5&	1&	0.5&	1&	0&	1&0  &	1\\
BGL         	&0.56&	0.96&	0.61&	0.94&	0.33&	0.96&	0.34&	0.3&	0.13&	0.96&	0.19&	0.94\\
Hadoop      	&0.57&	1&	0.5&	1&	0.46&	1&	0.44&	0.11&	0.29&	1&	0.19&	1\\
HDFS        	&1&	1&	1&	1&	0.4&	1&	0.5&	0&	0&	0&	1&	1  \\
HealthApp   	&0.96&	1&	0.92&	1&	0.55&	1&	0.5&	0.15&	0.48&	1&	1&	1\\
HPC         	&0.65&	1&	0.64&	1&	0.46&	1&	0.42&	0.28&	0.038&	1&	0.07&	1\\
Linux       	&0.57&	0.96&	0.59&	0.89&	0.35&	0.96&	0.33&	0.065&	0.29&	0.9&	0.28&	0.95\\
Mac         	&0.51&	0.95&	0.41&	0.957&	0.23&	0.97&	0.19&	0.15&	0.13&	0.91&	0.14&	0.93\\
OpenSSH     	&0.89&	1&	0.75&	1&	0.22&	1&	0.25&	0.12&	0.27&	1&	0.37&	1\\
OpenStack   	&0.66&	1&	0.66&	1&	0.66&	1&	0.66&	1&	0.33&	1&	0.33&	1\\
Spark       	&0.46&	1&	0.47&	1&	0.14&	1&	0.17&	0.3&	0.17&	1&	0.17&	1\\
Thunderbird 	&0.43&	0.95&	0.43&	0.94&	0.34&	0.98&	0.33&	0.13&	0.17&	0.95&	0.18&	0.94\\
Zookeeper   	&0.66&	1&	0.71&	1&	0.33&	1&	0.42&	0.14&	0.44&	1&	0.57&	1\\
\midrule
\textbf{Average} 
            &  &  &  &  &  &  &  &  &  &  &  & \\
\bottomrule
\end{tabular}}
\end{table}



==> figures/Table_complementory.tex <==
\begin{table}[!t]
\centering
\caption{Effect of augmentation on rare-log parsing across LLM-based parsers\anran{TPA denotes Template-Preserving Augmentation}}
\label{tab:rare_results}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Parser} & \textbf{PA} & \textbf{GA} & \textbf{FTA} & \textbf{FGA} \\
\midrule
EFParser + TPA  & 0.70 (4\%\gain{↑}) & \textbf{0.99} (2\%\gain{↑}) & 0.71 (5\%\gain{↑}) & \textbf{0.99}(1\%\gain{↑}) \\
LibreLog + TPA & 0.67 (13\%\gain{↑}) & 0.92 (1\%\drop{↓}) & 0.68 (15\%\gain{↑}) & 0.96 (17\%\gain{↑}) \\
LILAC-8shots + TPA & 0.55 (41\%\gain{↑}) & 0.93 (20\%\gain{↑}) & 0.55 (27\%\gain{↑}) & 0.94 (14\%\gain{↑}) \\

\bottomrule
\end{tabular}
}
\end{table} 

==> figures/abilation.tex <==
\begin{table*}[!t]
\centering
\caption{Impact of different setting on SEPLOG across log datasets.}
\label{tab:seplog_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccccccccc}
\toprule
Dataset & Metric & Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac & OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper \\
\midrule
\multirow{5}{*}{SEPLOG (Augmentation without pattern recognition)}
& PA  & 0   & 0.30 & 0.39 & 0.10 & --  & 0.34 & 0.57 & 0.31 & 0.22 & 0.66 & 0.21 & 0.40 & 0.50 &  \\
& GA  & 1   & 0.96 & 1    & 1    & --  & 1    & 0.94 & 0.92 & 1    & 1    & 1    & 0.96 & 1    &  \\
& FTA & 0   & 0.42 & 0.38 & 0.25 & --  & 0.35 & 0.53 & 0.32 & 0.25 & 0.66 & 0.27 & 0.40 & 0.50 & \\
& FGA & 1   & 0.94 & 1    & 1    & --  & 1    & 0.93 & 0.92 & 1    & 1    & 1    & 0.93 & 1 &   \\
& time & 0:01:13 & 0:23:19 & 0:31:04 & 1:06:40 & -- 
       & 0:09:47 & 0:4:21:56 & 6:59:01 & 0:10:53 & 0:21:52 
       & 0:18:42 & 15:39:27 & 1:09:23&  \\
\midrule
\multirow{5}{*}{SEPLOG (0-Augmentation)}
& PA  & 0.50 & 0.50 & 0.57 & 1    & 0.80 & 0.61 & 0.57 & 0.48 & 0.38 & 0.66 & 0.24 & 0.46 & 0.66 & \\
& GA  & 1    & 0.96 & 1    & 1    & 1    & 1    & 0.91 & 0.92 & 1    & 1    & 1    & 0.95 & 1  &   \\
& FTA & 0.50 & 0.57 & 0.45 & 1    & 0.68 & 0.57 & 0.71 & 0.43 & 0.37 & 0.66 & 0.27 & 0.47 & 0.71 & \\
& FGA & 1    & 0.94 & 1    & 1    & 0.82 & 1    & 0.93 & 0.93 & 1    & 1    & 1    & 0.95 & 1    & \\
& time & 00:00:04 & 00:02:07 & 00:01:20 & 00:00:08 & 00:00:33
       & 00:00:28 & 00:01:00 & 00:08:25 & 00:00:14 & 00:00:05
       & 00:00:38 & 02:57:52 & 00:01:44  &\\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/comparison_rare0.tex <==
\begin{table*}[!t]
\centering
\caption{Performance comparison of log parsers across datasets using PA, GA, FTA, and FGA metrics focusing on rare logs.}
\label{tab:parser_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccccccccccc|c}
\toprule
Method & Metric &
Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac &
OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper & Average \\
\midrule
\multirow{1}{*}{Total}
& \#log& 2 & 53 & 78 & 10 & 27 & 26 & 154 & 331 & 18 & 6 & 0.41 & 682 & 18 &1446  \\
\midrule
\multirow{4}{*}{SEPLOG}
& PA & \textbf{1} & 0.49 & 0.60 & \textbf{1} & \textbf{0.96} & 0.69 & \textbf{0.79} & \textbf{0.57} & 0.72 & 0.33 & \textbf{0.56} & \textbf{0.73} & \textbf{0.66} & 0.70 \\
& GA  & 1 & 0.96 & 1 & 1 & 1 & 1 & 0.90 & 0.91 & 0.61 & 1 & 0.90 & 0.86 & 1 & 0.96 \\
& FTA & 1 &\textbf{0.57} & \textbf{0.57} & 1 & 0.92 & \textbf{0.64} & \textbf{0.89} & 0.56 & \textbf{0.75} & 0.33 & \textbf{0.52} & \textbf{0.71} & 0.71 & 0.68 \\
& FGA & 1 & 0.94 & 1 & 1 & 1 & 1 & 0.93 & 0.91 & 1 & 1 & 1 & 0.97 & 1 &0.95  \\
\midrule
\multirow{4}{*}{Librelog}
& PA  & 0.50 & 0.41 & 0.60 & 0.80 & 0.88 & 0.46 & 0.70 & 0.48 & 0.44 & 0.66 & 0.46 & 0.53 & 0.66 &0.54  \\
& GA  & 1 & 0.96 & 1 & 1 & 1 & 1 & 0.90 & 0.91 & 1 & 1 & 1 & \textbf{0.98} & 1 & 0.81 \\
& FTA & 0.50 & 0.40 & 0.58 & 0.75 & 0.75 & 0.42 & 0.67 & 0.43 & 0.51 & 0.66 & 0.45 & 0.48 & 0.71 & 0.46 \\
& FGA & 1 & 0.94 & 1 & 0 & 0 & 0.28 & 0.89 & 0.92 & 0.80 & 1 & 0.30 & 0.90 & 1 & 0.84\\
\midrule
\multirow{4}{*}{LILAC}
& PA  & 0.50 & 0.52 & 0.43 & 0 & 0.96 & 0.07 & 0.08 & 0.29 & 0.11 & 0.66 & 0.41 & 0.37 & 0.66 &0.33  \\
& GA  & 1 & 0.86 & 0.88 & 1 & 1 & 0.23 & 0.1 & 0.85 & 0.5 & 1 & 0.90 & 0.80 & 1 & 0.82 \\
& FTA & 0.50 & 0.61 & 0.46 & 0 & 0.92 & 0.09 & 0.16 & 0.44 & 0.28 & 0.66 & 0.44 & 0.36 & 0.71 & 0.46 \\
& FGA & 1 & 0.88 & 0.84 & 1 & 1 & 0.27 & 0.24 & 0.93 & 0.71 & 1 & 0.93 & 0.85 & 1 & 0.87 \\
\midrule
\multirow{4}{*}{EFParser}
& PA  & 0.50 & 0.60 & 0.76 & 1& 0.88& 0.80 & 0.64 & 0.48 & 0.83 & 0.33 & 0.46 & 0.59 & 0.88 &0.59  \\
& GA  & 1 & 0.96 & 0.97 & 1 & 1 & 1 & 0.85 & 0.96 & 1 & 1 & 1 & 0.97 & 1 & 0.95 \\
& FTA & 0.50 & 0.64 & 0.73 & 1 & 0.76 & 0.78 & 0.67 & 0.48 & 0.87 & 0.33 & 0.52 & 0.61 & 0.85 & 0.59 \\
& FGA & 1 & 0.95 & 0.95 & 1 & 1 & 1 & 0.92 & 0.96 & 1 & 1 & 1 & 0.97 & 1 & 0.58 \\
\midrule
\multirow{4}{*}{Drain}
& PA  & 0 & 0.13 & 0.29 & 0 & 0.48 & 0.038 & 0.29 & 0.13 & 0.27 & 0.33 & 0.17 & 0.17 & 0.44 & 0.18 \\
& GA  & 1 & 0.96 & 1 & 0 & 1 & 1 & 0.9 & 0.91 & 1 & 1 & 1 & 0.95 & 1 & 0.94 \\
& FTA & 0 & 0.19 & 0.19 & 1 & 1 & 0.07 & 0.28 & 0.14 & 0.37 & 0.33 & 0.17 & 0.18 & 0.57 & 0.19 \\
& FGA & 1 & 0.94 & 1 & 1 & 1 & 1 & 0.95 & 0.93 & 1 & 1 & 1 & 0.94 & 1 & 0.93 \\
\midrule
\multirow{4}{*}{AEL}
& PA  & 0 & 0.20 & 0.46 & 0.80 & 0.48 & 0.03 & 0.27 & 0.16 & 0.27 & 0.66 & 0.21 & 0.19 & 0.44 &0.22  \\
& GA  & 1 & 0.83 & 0.92 & 1 & 1 & 1 & 0.79 & 0.92 & 1 & 1 & 1 & 0.97 & 1 & 0.92 \\
& FTA & 0 & 0.22 & 0.33 & 0.75 & 0.25 & 0.06 & 0.27 & 0.16 & 0.37 & 0.66 & 0.15 & 0.19 & 0.50 &0.20  \\
& FGA & 1 & 0.71 & 0.91 & 1 & 0.82 & 0.89 & 0.87 & 0.9 & 1 & 1 & 0.81 & 0.89 & 0.80 & 0.88 \\


\bottomrule



\end{tabular}
}
\end{table*}


==> figures/comparison_whole0.tex <==
\begin{table*}[!t]
\centering
\caption{Performance comparison of log parsers across datasets using PA, GA, FTA, and FGA metrics (entire datasets).}
\label{tab:parser_comparison_whole}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccccccccccc|c}
\toprule
Method & Metric &
Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac &
OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper & Average \\
\midrule
\multirow{4}{*}{SEPLOG}
& PA  & 0.99 & 0.91 & 0.84 & 1 & 0.97 & 0.94 & 0.88 & 0.70 & 0.68 & 0.78 & 0.85 & 0.78 & 0.95 & 0.86 \\
& GA  &1 & 0.92 & 0.93 & 1 & 0.99 & 0.84 & 0.96 & 0.90 & 0.70 & 0.78 & 0.88 & 0.88 & 0.99 & 0.92 \\
& FTA & 0.86 & 0.65 & 0.63 &0.82  & 0.79 & 0.64 & 0.59 & 0.65 & 0.67 & 0.44 & 0.68 & 0.35 & 0.83 & 0.56 \\
& FGA & 1 & 0.74 & 0.89 & 0.93 & 0.97 & 0.76 & 0.80 & 0.90 & 0.80 & 0.48 & 0.90 & 0.63 & 0.90 & 0.73 \\
\midrule
\multirow{4}{*}{Librelog}
& PA  & 0.99 & 0.95 & 0.74 & 0.97 & 0.94 & 0.92 & 0.75 & 0.66 & 0.27 & 0.76 & 0.88 & 0.63 & 0.84 &0.81  \\
& GA  & 0.99 & 0.91 & 0.94 & 0.94 & 0.86 & 0.79 & 0.81 & 0.86 & 0.61 & 0.77 & 0.88 & 0.73 & 0.99 & 0.81 \\
& FTA & 0.76 & 0.69 & 0.71 & 0.87 & 0.75 & 0.59 & 0.52 & 0.44 & 0.54 & 0.46 & 0.67 & 0.50 & 0.84 & 0.32 \\
& FGA & 0.94 & 0.79 & 0.92 & 0.90 & 0.94 & 0.70 & 0.78 & 0.78 & 0.68 & 0.47 & 0.88 & 0.83 & 0.98 &  0.59\\
\midrule
\multirow{4}{*}{LILAC}
& PA  & 0.97 & 0.82 & 0.58 & 0.83 & 0.66 & 0.86 & 0.61 & 0.42 & 0.9 & 0.91 & 0.86 & 0.38 & 0.37 & 0.68 \\
& GA  & 1 & 0.83 & 0.86 & 1 & 0.99 & 0.84 & 0.63 & 0.69 & 0.74 & 0.99 & 0.89 & 0.79 & 0.99 & 0.87 \\
& FTA & 0.72 & 0.66 & 0.44 & 0.44 & 0.67 & 0.59 & 0.49 & 0.38 & 0.5 & 0.69 & 0.58 & 0.11 & 0.71 & 0.54 \\
& FGA & 1 & 0.83 & 0.75 & 0.68 & 0.95 & 0.76 & 0.77 & 0.77 & 0.72 & 0.87 & 0.82 & 0.25 & 0.9 & 0.59 \\
\midrule
\multirow{4}{*}{EFParser}
& PA  & 0.99 & 0.97 & 0.75 & 0.66 & 0.94 & 0.98 & 0.36 & 0.58 & 0.94 & 0.96 & 0.87 & 0.69 & 0.84 & 0.77 \\
& GA  & 0.99 & 0.96& 0.94 & 1 & 0.99 & 0.85 & 0.39 & 0.92 & 0.69 & 0.98 & 0.83 & 0.83 & 0.99 & 0.88 \\
& FTA & 0.75 & 0.75 & 0.75 & 0.75 & 0.72 & 0.86 & 0.66 & 0.54 & 0.85 & 0.86 & 0.61 & 0.60 & 0.81 & 0.60 \\
& FGA & 0.91 & 0.88 & 0.93 & 0.96 & 0.93 & 0.88 & 0.88 & 0.90 & 0.80 & 0.96 & 0.82 & 0.83 & 0.88 & 0.86 \\
\midrule
\multirow{4}{*}{Drain}
& PA  & 0.72 & 0.4 & 0.54 & 0.62 & 0.31 & 0.72 & 0.11 & 0.35 & 0.58 & 0.03 & 0.39 & 0.21 & 0.84 & 0.46 \\
& GA  & 1 & 0.91 & 0.92 & 0.99 & 0.86 & 0.79 & 0.68 & 0.76 & 0.7 & 0.75 & 0.88 & 0.83 & 0.99 & 0.84 \\
& FTA & 0.51 & 0.19 & 0.38 & 0.6 & 0.4 & 0.15 & 0.25 & 0.7 & 0.48 & 0.002 & 0.41 & 0.07 & 0.61 & 0.28 \\
& FGA & 1 & 0.62 & 0.78 & 0.93 & 1 & 0.3 & 0.77 & 0.23 & 0.87 & 0.007 & 0.86 & 0.23 & 0.9 & 0.55 \\
\midrule
\multirow{4}{*}{AEL}
& PA  & 0.72 & 0.4 & 0.53 & 0.6 & 0.31 & 0.73 & 0.09 & 0.27 & 0.36 & 0.02 & - & 0.16 & 0.84 & 0.44 \\
& GA  & 1 & 0.95 & 0.95 & 0.99 & 0.96 & 0.95 & 0.95 & 0.9 & 0.7 & 0.27 & - & 0.78 & 0.98 & 0.85 \\
& FTA & 0.51 & 0.14 & 0.39 & 0.58 & 0.0017 & 0.11 & 0.23 & 0.2 & 0.44 & 0.2 & - & 0.35 & 0.62 & 0.25 \\
& FGA & 1 & 0.58 & 0.84 & 0.76 & 0.0081 & 0.27 & 0.77 & 0.79 & 0.88 & 0.6 & - & 0.11 & 0.76 & 0.55 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> figures/comparison_whole1.tex <==
\begin{table*}[!t]
\centering
\caption{Comparison of log parsers on full LogHub-2.0 datasets (excluding Proxifier)\fixme{Let's only present the average; new table (single column); rows as metrics, columns as baselines with SEPLOG on top; make the entire table available on Github}}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}}
& \multicolumn{4}{c|}{\textbf{SEPLOG}}
& \multicolumn{4}{c|}{\textbf{Librelog}}
& \multicolumn{4}{c|}{\textbf{LILAC-8shots}}
& \multicolumn{4}{c|}{\textbf{EFParser}}
& \multicolumn{4}{c|}{\textbf{Drain}}
& \multicolumn{4}{c}{\textbf{AEL}} \\
%\midrule
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA
& PA & GA & FTA & FGA \\
\midrule

Apache
& 0.99 & 1.00 & 0.86 & 1.00
& 0.99 & 0.99 & 0.76 & 0.94
& 0.97 & 1.00 & 0.72 & 1.00
& 0.99 & 0.99 & 0.75 & 0.91
& 0.72 & 1.00 & 0.51 & 1.00
& 0.72 & 1.00 & 0.51 & 1.00 \\

BGL
& 0.91 & 0.92 & 0.65 & 0.74
& 0.95 & 0.91 & 0.69 & 0.79
& 0.82 & 0.83 & 0.66 & 0.83
& 0.97 & 0.96 & 0.75 & 0.88
& 0.40 & 0.91 & 0.19 & 0.62
& 0.40 & 0.95 & 0.14 & 0.58 \\

Hadoop
& 0.84 & 0.93 & 0.63 & 0.89
& 0.74 & 0.94 & 0.71 & 0.92
& 0.58 & 0.86 & 0.44 & 0.75
& 0.75 & 0.94 & 0.75 & 0.93
& 0.54 & 0.92 & 0.38 & 0.78
& 0.53 & 0.95 & 0.39 & 0.84 \\

HDFS
& 1.00 & 1.00 & 0.82 & 0.93
& 0.97 & 0.94 & 0.87 & 0.90
& 0.83 & 1.00 & 0.44 & 0.68
& 0.66 & 1.00 & 0.75 & 0.96
& 0.62 & 0.99 & 0.60 & 0.93
& 0.60 & 0.99 & 0.58 & 0.76 \\

HealthApp
& 0.97 & 0.99 & 0.79 & 0.97
& 0.94 & 0.86 & 0.75 & 0.94
& 0.66 & 0.99 & 0.67 & 0.95
& 0.94 & 0.99 & 0.72 & 0.93
& 0.31 & 0.86 & 0.40 & 1.00
& 0.31 & 0.96 & <0.01 & <0.01 \\

HPC
& 0.94 & 0.84 & 0.64 & 0.76
& 0.92 & 0.79 & 0.59 & 0.70
& 0.86 & 0.84 & 0.59 & 0.76
& 0.98 & 0.85 & 0.86 & 0.88
& 0.72 & 0.79 & 0.15 & 0.30
& 0.73 & 0.95 & 0.11 & 0.27 \\

Linux
& 0.88 & 0.96 & 0.59 & 0.80
& 0.75 & 0.81 & 0.52 & 0.78
& 0.61 & 0.63 & 0.49 & 0.77
& 0.36 & 0.39 & 0.66 & 0.88
& 0.11 & 0.68 & 0.25 & 0.77
& 0.09 & 0.95 & 0.23 & 0.77 \\

Mac
& 0.70 & 0.90 & 0.65 & 0.90
& 0.66 & 0.86 & 0.44 & 0.78
& 0.42 & 0.69 & 0.38 & 0.77
& 0.58 & 0.92 & 0.54 & 0.90
& 0.35 & 0.76 & 0.70 & 0.23
& 0.27 & 0.90 & 0.20 & 0.79 \\

OpenSSH
& 0.68 & 0.70 & 0.67 & 0.80
& 0.27 & 0.61 & 0.54 & 0.68
& 0.90 & 0.74 & 0.50 & 0.72
& 0.94 & 0.69 & 0.85 & 0.80
& 0.58 & 0.70 & 0.48 & 0.87
& 0.36 & 0.70 & 0.44 & 0.88 \\

OpenStack
& 0.78 & 0.78 & 0.44 & 0.48
& 0.76 & 0.77 & 0.46 & 0.47
& 0.91 & 0.99 & 0.69 & 0.87
& 0.96 & 0.98 & 0.86 & 0.96
& 0.03 & 0.75 & 0.002 & 0.007
& 0.02 & 0.27 & 0.20 & 0.60 \\

Spark
& 0.85 & 0.88 & 0.68 & 0.90
& 0.88 & 0.88 & 0.67 & 0.88
& 0.86 & 0.89 & 0.58 & 0.82
& 0.87 & 0.83 & 0.61 & 0.82
& 0.39 & 0.88 & 0.41 & 0.86
& - & - & - & - \\

Thunderbird
& 0.78 & 0.88 & 0.50 & 0.63
& 0.63 & 0.73 & 0.50 & 0.83
& 0.38 & 0.79 & 0.11 & 0.25
& 0.69 & 0.83 & 0.60 & 0.83
& 0.21 & 0.83 & 0.07 & 0.23
& 0.16 & 0.78 & 0.35 & 0.11 \\

Zookeeper
& 0.95 & 0.99 & 0.83 & 0.90
& 0.84 & 0.99 & 0.84 & 0.98
& 0.37 & 0.99 & 0.71 & 0.90
& 0.84 & 0.99 & 0.81 & 0.88
& 0.84 & 0.99 & 0.61 & 0.90
& 0.84 & 0.98 & 0.62 & 0.76 \\
\midrule

Average
& \textbf{0.86} & \textbf{0.90} & 0.66 & 0.82
& 0.79 & 0.85 & 0.64 & 0.81
& 0.69 & 0.85 & 0.53 & 0.77
& 0.81 & 0.87 & \textbf{0.73} & \textbf{0.88}
& 0.44 & 0.86 & 0.26 & 0.54
& 0.38 & 0.79 & 0.29 & 0.56 \\

\bottomrule
\end{tabular}
}
\label{tab:parser_comparison-whole}
\end{table*}


==> figures/deprecated/freq-infreq.tex <==
\begin{table*}[!t]
\centering

\caption{Performance comparison on infrequent and frequent logs}
\label{tab:rare_freq_rowwise}
\resizebox{\linewidth}{!}{
%\begin{tabular}{ll|l|cccccccccccc|c}
\begin{tabular}{l|l|ccccccccccccc|c}
\toprule
%\textbf{Logs} & \textbf{Method} & \textbf{Metric} & Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac & OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper & Avg \\
\textbf{Method} & \textbf{Metric} & Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac & OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper & Avg \\
\midrule

%\multirow{12}{*}{Infrequent}
\multirow{4}{*}{LibreLog-INFreq}
&PA  & 0.5(48\%\drop{↓}) & 0.41 (56\%\drop{↓})& 0.60 (18\%\drop{↓})& 0.80(17\%\drop{↓}) & 0.88(6\%\drop{↓}) & 0.65(29\%\drop{↓}) & 0.70(6\%\drop{↓}) & 0.48(27\%\drop{↓})& 0.44(69\%\drop{↓}) & 0.66(13\%\drop{↓}) & 0.46(47\%\drop{↓}) & 0.53(15\%\drop{↓}) & 0.66(21\%\drop{↓}) &0.54(33\%\drop{↓}) \\
& GA  & 1(1\%\gain{↑}) & 0.96(5\%\gain{↑}) & 1(6\%\gain{↑}) & 1 (14\%\gain{↑})& 1(16\%\gain{↑}) & 1(26\%\gain{↑}) & 0.96(11\%\gain{↑}) & 0.95(5\%\gain{↑}) & 1(-) & 1(29\%\gain{↑}) & 1(2\%\gain{↑}) & 0.98(17\%\gain{↑}) & 1(1\%\gain{↑}) & 0.89(8\%\gain{↑}) \\
%&& FTA & 0.5(34\%\drop{↓}) & 0.40(42\%\drop{↓}) & 0.58(18\%\drop{↓}) & 0.75(12\%\drop{↓})& 0.75(13\%\drop{↓}) & 0.57(3\%\drop{↓}) & 0.67(28\%\gain{↑}) & 0.43(2\%\drop{↓}) & 0.51(5\%\drop{↓}) & 0.66(43\%\gain{↑}) & 0.45(32\%\drop{↓}) & 0.48(4\%\drop{↓}) & 0.71(15\%\drop{↓}) & 0.48(33\%\drop{↓})  \\
&FTA & 0.5 & 0.40& 0.58 & 0.75& 0.75 & 0.57 & 0.67 & 0.43& 0.51& 0.66 & 0.45 & 0.48 & 0.71 & 0.48  \\
%&& FGA & 1(6\%\gain{↑}) & 0.94(18\%\gain{↑}) & 1(8\%\gain{↑}) & 0(100\%\drop{↓}) & 1(6\%\gain{↑}) & 1(42\%\gain{↑}) & 0.89(14\%\gain{↑}) & 0.92(17\%\gain{↑}) & 0.80(17\%\gain{↑}) & 1(112\%\gain{↑}) & 0.30(65\%\drop{↓})& 0.90(8\%\gain{↑}) & 1(2\%\gain{↑}) & 0.87(52\%\gain{↑}) \\
&FGA & 1 & 0.94& 1 & 0 & 1 & 1 & 0.89 & 0.92 & 0.8 & 1 & 0.30& 0.90 & 1 & 0.87 \\
\midrule
\multirow{4}{*}{Drain-INFreq}
& PA  & 0(100\%\drop{↓}) & 0.13(67\%\drop{↓}) & 0.29(46\%\drop{↓}) & 0(100\%\drop{↓}) & 0.48(54\%\gain{↑}) & 0.03(95\%\drop{↓}) & 0.29(173\%\gain{↑}) & 0.13(62\%\drop{↓}) & 0.27(53\%\drop{↓}) & 0.33(15\%\gain{↑}) & 0.17(56\%\drop{↓}) & 0.17(19\%\drop{↓}) & 0.44(47\%\drop{↓}) & 0.18(52\%\drop{↓}) \\
& GA  & 1(1\%\gain{↑}) & 0.96(6\%\gain{↑}) & 1(4\%\gain{↑}) & 1(-) & 1(3\%\gain{↑}) & 1(11\%\gain{↑}) & 0.9(4\%\gain{↑}) & 0.91(12\%\gain{↑}) & 1(16\%\gain{↑}) & 1(20\%\gain{↑}) & 1(17\%\gain{↑}) & 0.95(10\%\gain{↑}) & 1(19\%\gain{↑}) & 0.94(5\%\gain{↑}) \\
%&& FTA & 0.18(-) & 1(-) & 0.14(87\%\drop{↓}) & 0.33(-) & 0.17(70\%\gain{↑})& 1(-) & 0.19(19\%\gain{↑}) & 0(100\%\drop{↓}) & 0.28(41\%\gain{↑}) & 0.57(19\%\gain{↑})& 0.07(-) & 0.19(26\%\gain{↑}) & 0.37(13\%\gain{↑}) & 0.19(180\%\gain{↑}) \\
&FTA & 0.18 & 1 & 0.14 & 0.33& 0.17& 1 & 0.19 & 0 & 0.28 & 0.57& 0.07 & 0.19 & 0.37 & 0.19 \\
%&& FGA & 0.94(6\%\drop{↓}) & 1(65\%\gain{↑}) & 0.93(23\%\gain{↑}) & 1(5\%\drop{↓}) & 1(106\%\gain{↑}) & 1(92\%\gain{↑}) & 1(35\%\gain{↑}) & 1(200\%\gain{↑}) & 0.95(27\%\gain{↑}) & 1(23\%\gain{↑}) & 1(30\%\drop{↓}) & 0.94(30\%\gain{↑}) & 1(11\%\gain{↑}) & 0.93(8\%\gain{↑}) \\
&FGA & 0.94 & 1 & 0.93 & 1 & 1 & 1 & 1 & 1 & 0.95 & 1 & 1 & 0.94 & 1 & 0.93 \\
\midrule
\multirow{4}{*}{LILAC-INFreq}
& PA  & 0.5(48\%\drop{↓}) & 0.52(36\%\drop{↓}) & 0.43(25\%\drop{↓}) & 0(100\%\drop{↓}) & 0.96(45\%\gain{↑}) & 0.07(90\%\drop{↓}) & 0.08(86\%\drop{↓}) & 0.29(31\%\drop{↓}) & 0.11(87\%\drop{↓}) & 0.66(27\%\drop{↓}) & 0.41(52\%\drop{↓}) & 0.37(2\%\drop{↓}) & 0.66(78\%\gain{↑}) & 0.33(51\%\drop{↓}) \\
& GA  & 1(-) & 0.86(3\%\gain{↑}) & 0.88(2\%\gain{↑}) & 1(-) & 1(1\%\gain{↑}) & 0.23(72\%\drop{↓}) & 0.1(84\%\drop{↓}) & 0.85(23\%\gain{↑}) & 0.5(32\%\drop{↓}) & 1(10\%\gain{↑}) & 0.9(11\%\gain{↑}) & 0.8(12\%\gain{↑}) & 1(10\%\gain{↑}) & 0.82(5\%\drop{↓}) \\
%&& FTA & 0.5(32\%\drop{↓}) & 0.61(8\%\drop{↓}) & 0.46(5\%\gain{↑}) & 0(100\%\drop{↓}) & 0.92(41\%\gain{↑}) & 0.09(86\%\drop{↓}) & 0.16(68\%\drop{↓}) & 0.44(126\%\gain{↑}) & 0.28(49\%\drop{↓}) & 0.66(4\%\drop{↓}) & 0.44(25\%\drop{↓}) & 0.36(-) & 0.71(-) & 0.46(360\%\gain{↑}) \\
&FTA & 0.5 & 0.61 & 0.46 & 0 & 0.92 & 0.09 & 0.16 & 0.44 & 0.28 & 0.66 & 0.44 & 0.36 & 0.71 & 0.46\\
%&& FGA & 1(-) & 0.88(6\%\gain{↑}) & 0.84(14\%\gain{↑}) & 1(52\%\gain{↑}) & 1(6\%\gain{↑}) & 0.27(8\%\drop{↓}) & 0.24(8\%\drop{↓}) & 0.93(340\%\gain{↑}) & 0.71(8\%\drop{↓}) & 1(17\%\gain{↑}) & 0.93(15\%\gain{↑}) & 0.85(720\%\gain{↑}) & 1(13\%\gain{↑}) & 0.87(260\%\gain{↑}) \\
&FGA & 1 & 0.88 & 0.84 & 1 & 1 & 0.27 & 0.24 & 0.93 & 0.71 & 1 & 0.93 & 0.85 & 1 & 0.87 \\

\midrule

%\multirow{12}{*}{Frequent}
\multirow{4}{*}{LibreLog-Freq}
& PA  & 0.98 & 0.95 & 0.74 & 0.97 & 0.94 & 0.92 & 0.75 & 0.66 & 0.26 & 0.76 & 0.88 & 0.63 & 0.84 & 0.81 \\
& GA  & 0.99 & 0.91 & 0.94 & 0.87 & 0.86 & 0.79 & 0.81 & 0.86 & 0.61 & 0.77 & 0.88 & 0.73 & 0.99 & 0.82 \\
& FTA & 0.76 & 0.69 & 0.71 & 0.86 & 0.87 & 0.59 & 0.52 & 0.44 & 0.54 & 0.46 & 0.67 & 0.5 & 0.84 & 0.72 \\
& FGA & 0.94 & 0.79 & 0.92 & 0.75 & 0.94 & 0.7 & 0.78 & 0.78 & 0.68 & 0.47 & 0.88 & 0.83 & 0.98 & 0.57 \\
\midrule
\multirow{4}{*}{Drain-Freq}
& PA  & 0.72 & 0.40 & 0.54 & 0.62 & 0.31 & 0.72 & 0.11 & 0.35 & 0.58 & 0.02 & 0.39 & 0.21 & 0.84 & 0.38 \\
& GA  & 0.99 & 0.90 & 0.96 & 1.00 & 0.97 & 0.90 & 0.86 & 0.81 & 0.86 & 0.83 & 0.85 & 0.86 & 0.84 & 0.89 \\
& FTA & 0.18 & 1.00 & 1.11 & 0.33 & 0.10 & 1.00 & 0.16 & 0.00 & 0.20 & 0.48 & 0.07 & 0.15 & 0.33 & 0.18 \\
& FGA & 1.00 & 0.60 & 0.75 & 1.06 & 0.01 & 0.52 & 0.74 & 0.31 & 0.03 & 0.04 & 1.45 & 0.23 & 0.89 & 0.10 \\
\midrule
\multirow{4}{*}{LILAC-Freq}
& PA  & 0.97 & 0.82 & 0.58 & 0.83 & 0.66 & 0.73 & 0.61 & 0.42 & 0.90 & 0.91 & 0.86 & 0.38 & 0.37 & 0.68 \\
& GA  & 1.00 & 0.83 & 0.86 & 1.00 & 0.99 & 0.84 & 0.63 & 0.69 & 0.74 & 0.99 & 0.89 & 0.79 & 0.99 & 0.87 \\
& FTA & 0.74 & 0.66 & 0.44 & 0.49 & 0.65 & 0.67 & 0.50 & 0.44 & 0.55 & 0.69 & 0.59 & 0.36 & 0.71 & 0.10 \\
& FGA & 1.00 & 0.83 & 0.73 & 0.66 & 0.94 & 0.86 & 0.84 & 0.21 & 0.73 & 0.85 & 0.80 & 0.10 & 0.88 & 0.24 \\

\bottomrule
\end{tabular}
}
\end{table*}



==> figures/empirical/sota0.tex <==
\begin{table*}[!t]
\centering

\caption{Performance comparison on rare and frequent logs}
\label{tab:rare_freq_rowwise}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccccccccccc|c}
\toprule
\textbf{Method} & \textbf{Metric} & Apache & BGL & Hadoop & HDFS & HealthApp & HPC & Linux & Mac & OpenSSH & OpenStack & Spark & Thunderbird & Zookeeper & Avg \\
\midrule

%\multirow{12}{*}{Infrequent}
\multirow{4}{*}{LibreLog-INFreq}
&PA  & 0.5(48\%\drop{↓}) & 0.41 (56\%\drop{↓})& 0.60 (18\%\drop{↓})& 0.80(17\%\drop{↓}) & 0.88(6\%\drop{↓}) & 0.65(29\%\drop{↓}) & 0.70(6\%\drop{↓}) & 0.48(27\%\drop{↓})& 0.44(69\%\drop{↓}) & 0.66(13\%\drop{↓}) & 0.46(47\%\drop{↓}) & 0.53(15\%\drop{↓}) & 0.66(21\%\drop{↓}) &0.54(33\%\drop{↓}) \\
& GA  & 1(1\%\gain{↑}) & 0.96(5\%\gain{↑}) & 1(6\%\gain{↑}) & 1 (14\%\gain{↑})& 1(16\%\gain{↑}) & 1(26\%\gain{↑}) & 0.96(11\%\gain{↑}) & 0.95(5\%\gain{↑}) & 1(-) & 1(29\%\gain{↑}) & 1(2\%\gain{↑}) & 0.98(17\%\gain{↑}) & 1(1\%\gain{↑}) & 0.89(8\%\gain{↑}) \\
%&& FTA & 0.5(34\%\drop{↓}) & 0.40(42\%\drop{↓}) & 0.58(18\%\drop{↓}) & 0.75(12\%\drop{↓})& 0.75(13\%\drop{↓}) & 0.57(3\%\drop{↓}) & 0.67(28\%\gain{↑}) & 0.43(2\%\drop{↓}) & 0.51(5\%\drop{↓}) & 0.66(43\%\gain{↑}) & 0.45(32\%\drop{↓}) & 0.48(4\%\drop{↓}) & 0.71(15\%\drop{↓}) & 0.48(33\%\drop{↓})  \\
&FTA & 0.5 & 0.40& 0.58 & 0.75& 0.75 & 0.57 & 0.67 & 0.43& 0.51& 0.66 & 0.45 & 0.48 & 0.71 & 0.48  \\
%&& FGA & 1(6\%\gain{↑}) & 0.94(18\%\gain{↑}) & 1(8\%\gain{↑}) & 0(100\%\drop{↓}) & 1(6\%\gain{↑}) & 1(42\%\gain{↑}) & 0.89(14\%\gain{↑}) & 0.92(17\%\gain{↑}) & 0.80(17\%\gain{↑}) & 1(112\%\gain{↑}) & 0.30(65\%\drop{↓})& 0.90(8\%\gain{↑}) & 1(2\%\gain{↑}) & 0.87(52\%\gain{↑}) \\
&FGA & 1 & 0.94& 1 & 0 & 1 & 1 & 0.89 & 0.92 & 0.8 & 1 & 0.30& 0.90 & 1 & 0.87 \\
\midrule
\multirow{4}{*}{Drain-INFreq}
& PA  & 0(100\%\drop{↓}) & 0.13(67\%\drop{↓}) & 0.29(46\%\drop{↓}) & 0(100\%\drop{↓}) & 0.48(54\%\gain{↑}) & 0.03(95\%\drop{↓}) & 0.29(173\%\gain{↑}) & 0.13(62\%\drop{↓}) & 0.27(53\%\drop{↓}) & 0.33(15\%\gain{↑}) & 0.17(56\%\drop{↓}) & 0.17(19\%\drop{↓}) & 0.44(47\%\drop{↓}) & 0.18(52\%\drop{↓}) \\
& GA  & 1(1\%\gain{↑}) & 0.96(6\%\gain{↑}) & 1(4\%\gain{↑}) & 1(-) & 1(3\%\gain{↑}) & 1(11\%\gain{↑}) & 0.9(4\%\gain{↑}) & 0.91(12\%\gain{↑}) & 1(16\%\gain{↑}) & 1(20\%\gain{↑}) & 1(17\%\gain{↑}) & 0.95(10\%\gain{↑}) & 1(19\%\gain{↑}) & 0.94(5\%\gain{↑}) \\
%&& FTA & 0.18(-) & 1(-) & 0.14(87\%\drop{↓}) & 0.33(-) & 0.17(70\%\gain{↑})& 1(-) & 0.19(19\%\gain{↑}) & 0(100\%\drop{↓}) & 0.28(41\%\gain{↑}) & 0.57(19\%\gain{↑})& 0.07(-) & 0.19(26\%\gain{↑}) & 0.37(13\%\gain{↑}) & 0.19(180\%\gain{↑}) \\
&FTA & 0.18 & 1 & 0.14 & 0.33& 0.17& 1 & 0.19 & 0 & 0.28 & 0.57& 0.07 & 0.19 & 0.37 & 0.19 \\
%&& FGA & 0.94(6\%\drop{↓}) & 1(65\%\gain{↑}) & 0.93(23\%\gain{↑}) & 1(5\%\drop{↓}) & 1(106\%\gain{↑}) & 1(92\%\gain{↑}) & 1(35\%\gain{↑}) & 1(200\%\gain{↑}) & 0.95(27\%\gain{↑}) & 1(23\%\gain{↑}) & 1(30\%\drop{↓}) & 0.94(30\%\gain{↑}) & 1(11\%\gain{↑}) & 0.93(8\%\gain{↑}) \\
&FGA & 0.94 & 1 & 0.93 & 1 & 1 & 1 & 1 & 1 & 0.95 & 1 & 1 & 0.94 & 1 & 0.93 \\
\midrule
\multirow{4}{*}{LILAC-INFreq}
& PA  & 0.5(48\%\drop{↓}) & 0.52(36\%\drop{↓}) & 0.43(25\%\drop{↓}) & 0(100\%\drop{↓}) & 0.96(45\%\gain{↑}) & 0.07(90\%\drop{↓}) & 0.08(86\%\drop{↓}) & 0.29(31\%\drop{↓}) & 0.11(87\%\drop{↓}) & 0.66(27\%\drop{↓}) & 0.41(52\%\drop{↓}) & 0.37(2\%\drop{↓}) & 0.66(78\%\gain{↑}) & 0.33(51\%\drop{↓}) \\
& GA  & 1(-) & 0.86(3\%\gain{↑}) & 0.88(2\%\gain{↑}) & 1(-) & 1(1\%\gain{↑}) & 0.23(72\%\drop{↓}) & 0.1(84\%\drop{↓}) & 0.85(23\%\gain{↑}) & 0.5(32\%\drop{↓}) & 1(10\%\gain{↑}) & 0.9(11\%\gain{↑}) & 0.8(12\%\gain{↑}) & 1(10\%\gain{↑}) & 0.82(5\%\drop{↓}) \\
%&& FTA & 0.5(32\%\drop{↓}) & 0.61(8\%\drop{↓}) & 0.46(5\%\gain{↑}) & 0(100\%\drop{↓}) & 0.92(41\%\gain{↑}) & 0.09(86\%\drop{↓}) & 0.16(68\%\drop{↓}) & 0.44(126\%\gain{↑}) & 0.28(49\%\drop{↓}) & 0.66(4\%\drop{↓}) & 0.44(25\%\drop{↓}) & 0.36(-) & 0.71(-) & 0.46(360\%\gain{↑}) \\
&FTA & 0.5 & 0.61 & 0.46 & 0 & 0.92 & 0.09 & 0.16 & 0.44 & 0.28 & 0.66 & 0.44 & 0.36 & 0.71 & 0.46\\
%&& FGA & 1(-) & 0.88(6\%\gain{↑}) & 0.84(14\%\gain{↑}) & 1(52\%\gain{↑}) & 1(6\%\gain{↑}) & 0.27(8\%\drop{↓}) & 0.24(8\%\drop{↓}) & 0.93(340\%\gain{↑}) & 0.71(8\%\drop{↓}) & 1(17\%\gain{↑}) & 0.93(15\%\gain{↑}) & 0.85(720\%\gain{↑}) & 1(13\%\gain{↑}) & 0.87(260\%\gain{↑}) \\
&FGA & 1 & 0.88 & 0.84 & 1 & 1 & 0.27 & 0.24 & 0.93 & 0.71 & 1 & 0.93 & 0.85 & 1 & 0.87 \\

\midrule

%\multirow{12}{*}{Frequent}
\multirow{4}{*}{LibreLog-Freq}
& PA  & 0.98 & 0.95 & 0.74 & 0.97 & 0.94 & 0.92 & 0.75 & 0.66 & 0.26 & 0.76 & 0.88 & 0.63 & 0.84 & 0.81 \\
& GA  & 0.99 & 0.91 & 0.94 & 0.87 & 0.86 & 0.79 & 0.81 & 0.86 & 0.61 & 0.77 & 0.88 & 0.73 & 0.99 & 0.82 \\
& FTA & 0.76 & 0.69 & 0.71 & 0.86 & 0.87 & 0.59 & 0.52 & 0.44 & 0.54 & 0.46 & 0.67 & 0.5 & 0.84 & 0.72 \\
& FGA & 0.94 & 0.79 & 0.92 & 0.75 & 0.94 & 0.7 & 0.78 & 0.78 & 0.68 & 0.47 & 0.88 & 0.83 & 0.98 & 0.57 \\
\midrule
\multirow{4}{*}{Drain-Freq}
& PA  & 0.72 & 0.40 & 0.54 & 0.62 & 0.31 & 0.72 & 0.11 & 0.35 & 0.58 & 0.02 & 0.39 & 0.21 & 0.84 & 0.38 \\
& GA  & 0.99 & 0.90 & 0.96 & 1.00 & 0.97 & 0.90 & 0.86 & 0.81 & 0.86 & 0.83 & 0.85 & 0.86 & 0.84 & 0.89 \\
& FTA & 0.18 & 1.00 & 1.11 & 0.33 & 0.10 & 1.00 & 0.16 & 0.00 & 0.20 & 0.48 & 0.07 & 0.15 & 0.33 & 0.18 \\
& FGA & 1.00 & 0.60 & 0.75 & 1.06 & 0.01 & 0.52 & 0.74 & 0.31 & 0.03 & 0.04 & 1.45 & 0.23 & 0.89 & 0.10 \\
\midrule
\multirow{4}{*}{LILAC-Freq}
& PA  & 0.97 & 0.82 & 0.58 & 0.83 & 0.66 & 0.73 & 0.61 & 0.42 & 0.90 & 0.91 & 0.86 & 0.38 & 0.37 & 0.68 \\
& GA  & 1.00 & 0.83 & 0.86 & 1.00 & 0.99 & 0.84 & 0.63 & 0.69 & 0.74 & 0.99 & 0.89 & 0.79 & 0.99 & 0.87 \\
& FTA & 0.74 & 0.66 & 0.44 & 0.49 & 0.65 & 0.67 & 0.50 & 0.44 & 0.55 & 0.69 & 0.59 & 0.36 & 0.71 & 0.10 \\
& FGA & 1.00 & 0.83 & 0.73 & 0.66 & 0.94 & 0.86 & 0.84 & 0.21 & 0.73 & 0.85 & 0.80 & 0.10 & 0.88 & 0.24 \\

\bottomrule
\end{tabular}
}
\end{table*}



==> figures/llms.tex <==
\begin{table}[!t]
\centering
\caption{Performance comparison of different LLMs}
\label{tab:llm_comparison}
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{2cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
\textbf{Model} & \textbf{PA} & \textbf{GA} & \textbf{FTA} & \textbf{FGA} \\
\midrule
Llama3-8B & 0.80 & 0.97 & 0.80 & 0.97 \\
Mistral-7B & 0.70 (12\%\drop{↓}) & 0.92 (5\%\drop{↓})& 0.77 (3\%\drop{↓})& 0.93 (4\%\drop{↓}) \\
Gemma-2-9b-it & 0.80 (-) & 0.99 (2\%\gain{↑}) & 0.80 (-) & 0.98 (1\%\gain{↑}) \\
\bottomrule
\end{tabular}
}
\end{table}



==> sections/Discussion.tex <==
\section{Discussion}
The results demonstrate that the proposed augmentation and diversity-guided sampling strategies improve template inference robustness under long-tailed log distributions. In particular, exposing the parser to structurally diverse yet template-consistent examples helps the LLM more reliably distinguish structural tokens from dynamic tokens, especially for rare log groups. However, the improvements are not uniform across all datasets, suggesting that augmentation effectiveness depends on dataset characteristics such as template diversity and structural variability.

The statistical analysis further confirms that these improvements are unlikely to be caused by random variation across datasets, providing additional evidence that the proposed augmentation strategy contributes to more robust template inference.

The findings also highlight the importance of preserving semantic and structural consistency during augmentation. Augmenting log messages without first abstracting dynamic tokens can introduce unrealistic token variations that distort the underlying template structure and negatively affect template inference. This suggests that effective augmentation requires not only increasing the number of examples but also ensuring that generated examples remain structurally consistent with the original template. Future work could investigate adaptive augmentation strategies that dynamically adjust augmentation behavior according to dataset characteristics.

The results further suggest that the proposed augmentation strategy is complementary to existing LLM-based parsers. Since it operates only during in-context example construction and does not modify the underlying parsing architecture, it can be integrated into existing frameworks without changing their core design. The consistent improvements observed across multiple state-of-the-art parsers indicate that augmentation serves as a general mechanism for improving robustness under highly imbalanced log distributions rather than a parser-specific optimization.


==> sections/Experiment_setup.tex <==
\section{Experiment setup}

This section describes the experimental configuration used to evaluate our approach, including the dataset, execution environment, implementation details, and evaluation metrics.
Dataset Description
We conduct our experiments on LogHub-2.0, a large-scale benchmark dataset widely used for evaluating log parsing techniques. The dataset consists of log messages collected from 14 open-source systems spanning multiple application domains, including distributed systems, supercomputing environments, and server-side applications. Due to its diversity and the availability of ground-truth annotations, LogHub has become a standard benchmark for reproducible log parsing evaluation.
Compared to its predecessor, LogHub-2.0 significantly increases both scale and complexity. It contains more than 50 million log messages corresponding to 3,488 unique ground-truth templates, with each log message explicitly labeled by its originating template. This scale enables systematic evaluation of parsing accuracy across both frequent and rare log patterns, which is essential for assessing real-world robustness.

\textbf{Experimental Environment and Implementation}
All experiments are executed on a Linux-based server environment. The implementations are developed and run using Python 3.9. To ensure fair comparison, all baseline methods are evaluated under the same execution environment using their default configurations unless otherwise specified.
For LLM-based parsing, we evaluate \tool using three open-source large language models: LLaMA-3.8B, CodeGemma-7B, and Misteral-7B . These model are selected to represent oprn source modern, lightweight LLMs that balance reasoning capability with computational efficiency, making them suitable for large-scale log parsing on shared server infrastructure. To ensure deterministic behavior and improve output stability, the temperature parameter is fixed to 0 during inference. Although our experiments focus on these three models, the framework itself is model-agnostic and can be readily extended to other LLM backbones.

\textbf{Evaluation Metrics}
We evaluate log parsing performance using four complementary metrics that capture both log-level and template-level correctness: Parsing Accuracy (PA), Grouping Accuracy (GA), F1-score of template Accuracy (FTA), and F1-score of Group Accuracy(FGA).
Parsing Accuracy (PA).
PA measures whether individual log messages are parsed exactly according to their ground-truth templates. A log message is considered correctly parsed only if both its static components and dynamic variables exactly match the ground truth. PA is defined as the ratio of correctly parsed log messages to the total number of log messages, providing a strict assessment of parsing correctness at the log-message level.
Grouping Accuracy (GA).
GA evaluates the ability of a parser to correctly group log messages originating from the same ground-truth template. A log message is considered correctly grouped if it is assigned to a group that contains exactly the same set of messages as its underlying template. GA is computed as the proportion of correctly grouped log messages among all log messages. While GA captures grouping consistency, it does not verify the correctness of the extracted templates.
F1-score of Template Accuracy (FTA).
FTA assesses parsing correctness at the template level. A predicted template is regarded as correct if and only if all log messages assigned to it originate from a single ground-truth template and the static tokens of the predicted template exactly match those of the ground truth. FTA is computed as the ratio of correctly identified templates to the total number of predicted templates. This metric penalizes over-generalized or incorrectly extracted templates that may otherwise achieve high log-level accuracy.
F1-score of Group Accuracy (FGA).
FGA evaluates grouping performance at the template level. A predicted template is considered correctly grouped if the set of log messages assigned to it exactly matches the set of messages associated with a ground-truth template. FGA is defined as the harmonic mean of precision and recall computed over correctly grouped templates.
Together, these metrics provide a comprehensive evaluation of log parsing performance, capturing both fine-grained correctness and structural grouping behavior.



==> sections/Introduction-old.tex <==
\section{Introduction}


%\note{Always use reference tag, e.g., Section~\ref{section2} instead of Section~2}
\anran{Paragraph 1: Logs are important. Log parsing enables downstream analysis.}
\fixme{Software systems continuously generate large volumes of logs during execution.}

\anran{Paragraph 2: Modern parsers work well overall.}
\fixme{Existing log parsers, ranging from heuristic-based methods to recent LLM-based approaches, have substantially improved template inference across diverse logging systems.}

\anran{Paragraph 3: But they struggle on rare log groups because of limited structural evidence.}
\fixme{Despite these advances, state-of-the-art parsers can still fail completely on log templates that appear only a handful of times in practice. Table~\ref{} shows an example from the Mac dataset.}

\anran{Paragraph 4: Explain the root cause and research gap}
\fixme{The underlying challenge is that real-world log datasets exhibit highly imbalanced, long-tailed distributions, where rare log groups provide insufficient structural evidence for reliable template inference. [..] Although rare log groups are operationally important, their prevalence, impact on parser robustness, and influence on current evaluation practices remain largely unexplored.}

\anran{Paragraph 5: We study this problem}
\fixme{To better understand this challenge, we conduct a large-scale empirical study on Loghub-2.0. [..] These findings motivate approaches that explicitly address the lack of structural evidence.}

\anran{Paragraph 6: We propose \tool to address it. \tool's high-level overview}
\fixme{To address this challenge, we propose \tool, a template-preserving augmentation framework that improves template inference by enriching rare log groups before parsing. The key idea behind TRAIL is that rare log groups fail not because existing parsers lack semantic reasoning, but because they lack sufficient structural evidence. Describe \tool's pipeline here.}

\anran{Paragraph 7: Contributions}
\fixme{In summary, this paper makes the following contributions:}

Software systems continuously generate large volumes of logs during execution. These logs provide detailed records of runtime events, system states, warnings, and failures, capturing valuable information about system behavior. The collection and examination of such logs, commonly referred to as log analysis, play a critical role in many software engineering activities. These include software debugging ~\cite{xu2009detecting,Yuan2010Sherlog,chen2019empirical,chen2021pathidea}, system monitoring ~\cite{Wang2021QuickPeek,Chen2019LoadTests,candido2021logbased,razavi2008pattern}, anomaly detection ~\cite{Chen2019LoadTests,he2017towards,Su2024LLMForecasting,LibreLog2024,huo2023semparser,Zhang2020UnstableLogs,he2016loganalysis,sun2026improving}, failure prediction ~\cite{das2020failure,lim2008log,zheng2009system,zhang2016automated}, and root cause analysis ~\cite{lu2017logbased,zawawy2010log,suriadi2012root,mariani2008automated}. As software systems become increasingly complex, developers rely heavily on automated log analysis techniques to maintain system reliability and availability.
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figures/log_parsing_example.pdf}
    \caption{Example of log parsing from the Linux dataset.}
    \label{fig:logexample}
\end{figure}
Logs consist of individual log messages, which are generated when logging statements embedded in source code are executed. A logging statement typically contains a fixed textual structure describing an event and one or more runtime variables whose values are instantiated during execution. Consequently, log messages are inherently semi-structured: messages generated from the same logging statement share a common structure while differing in their variable content. Figure~\ref{fig:logexample} presents examples of log messages from the Linux dataset. The first two raw log messages are generated from the same logging statement and therefore correspond to the same log template. They contain identical static text describing the event, while the values highlighted as parameters represent dynamic content that varies across executions. 
% \sepideh{we dont have third one}In contrast, the third message originates from a different logging statement and thus corresponds to a different template. 
This semi-structured nature allows developers to identify recurring execution templates, but dynamic variables make automated analysis challenging.

To facilitate downstream log analytics tasks, raw log messages are typically transformed into structured representations through a process known as log parsing. Log parsing identifies the static tokens shared among similar messages and extracts the dynamic parameters, producing a generalized log template for each group of related messages. These structured templates serve as the foundation for many subsequent log analysis tasks, including anomaly detection, failure prediction, and root cause analysis.

Traditional log parsers, such as Drain ~\cite{Drain2017} and Spell ~\cite{Spell2019}, rely on heuristic rules, token matching, or tree-based structures to identify templates. These methods are computationally efficient and perform well when log formats are repetitive and consistent. More recently, large language model (LLM)-based parsers, such as LibreLog ~\cite{LibreLog2024}, LILAC~\cite{LILAC2024}, and EFParser~\cite{wang2026small}, have demonstrated promising performance by leveraging semantic understanding to infer template structures from log messages. Compared with rule-based approaches, LLM-based parsers are generally more flexible and better equipped to handle diverse logging formats. Nevertheless, their effectiveness often depends on the availability of sufficient examples from which template structures can be inferred.

\input{figures/Motivation_example}
In practice, however, log datasets are highly imbalanced. A small number of templates typically account for the majority of log messages, while many templates appear only a few times. This phenomenon arises naturally because common system behaviors generate logs repeatedly, whereas critical system behaviors such as failures, exceptional events, and uncommon execution paths occur rarely. As a result, frequent templates provide abundant structural evidence for template inference, while rare templates are represented by only a handful of examples. Failing to parse these rare logs correctly may hide infrequent but operationally critical behaviors, such as failures and exceptional events, from downstream analysis.

Recent work by Jiang et al. ~\cite{jiang2024large}  showed that parser performance varies substantially across template frequencies and that rare templates remain particularly challenging to parse.
We observe the same trend across Loghub-2.0, as discussed in Section~\ref{section2}.
Table ~\ref{tab:example} presents a motivating example from the Mac dataset. LibreLog~\cite{LibreLog2024}, a state-of-the-art LLM-based parser, achieves perfect parsing accuracy on template E113, which accounts for 7.7\% of all log messages. In contrast, its accuracy drops to 0\% on template E164, which appears only three times in the dataset. This example illustrates how limited structural evidence can hinder accurate template inference for underrepresented log groups.

%\anran{to fix}
Despite the success of recent LLM-based parsers, it remains unclear how prevalent rare log groups are in real-world datasets, how much they affect parser performance, and whether existing evaluation metrics accurately capture parser robustness under highly imbalanced log distributions.

To answer these questions, we conduct a large-scale empirical study on Loghub-2.0. Our results show that rare log groups constitute a substantial proportion of templates despite representing only a tiny fraction of log messages. Existing parsers degrade considerably on these groups, and commonly used evaluation metrics can overestimate parser robustness because frequent log groups dominate overall evaluation results. These findings indicate that improving parser robustness requires explicitly addressing underrepresented log groups rather than relying only on existing template inference strategies.

Motivated by these findings, we propose \tool, a rare-log-aware parsing framework designed to improve robustness under imbalanced log distributions. \tool augments underrepresented log groups before template inference, providing richer structural evidence for identifying static tokens and dynamic variables. Experimental results show that \tool consistently improves parsing accuracy on rare log groups and achieves up to 19.4\% improvement over the strongest baseline while maintaining competitive performance on complete datasets.

In short, this paper makes the following key contributions:
\begin{itemize}
    \item To the best of our knowledge, we are the first to study the prevalence of rare logs and its impact on log parsing. We show that existing log parsing evaluations can overestimate parser robustness by masking performance degradation on rare log groups.
    \item We introduce \tool, an augmentation-driven framework designed to improve the robustness of state-of-the-art log parsers under imbalanced log distributions.
    \item We demonstrate the generalizability of our augmentation strategy by improving state-of-the-art LLM-based parsers while preserving their original designs.
    % \item We present the one of the first large-scale empirical study on the impact of long-tailed log distributions on log parsing. Across 13 datasets containing over 50 million log messages, we show that real-world logs exhibit severe imbalance, which significantly affects the robustness of existing parsers.
    % \item We re-evaluate five state-of-the-art log parsers under long-tailed settings and show that their performance degrades substantially on rare log groups.
    % \item We propose \tool, a rare-group enhancement log parsing framework designed for long-tailed log distributions. It strengthens rare log groups through semantic template generation, log augmentation, and diversity sampling to enable reliable template inference under highly imbalanced data.
    \item To facilitate future research, we make our replication package publicly available at \url{https://anonymous.4open.science/r/TRAIL-parser-6A5F/}.
\end{itemize}


% The rest of this paper is organized as follows. Section~2 presents the empirical study on rare logs. Section~3 presents our proposed approach. Section~4 presents our study design. Section~5 describes the experimental setup and results. Section~6 presents threats to validity. Section~7 reviews related work. Section~8 presents the discussion. Finally, Section~9 concludes the paper.



\begin{figure*}[t]
\centering

% Row 1
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/Thunderbird_log_distribution.pdf}
\\(a) Thunderbird
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/Mac_log_distribution.pdf}
\\(b) Mac
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/BGL_log_distribution.pdf}
\\(c) BGL
\end{minipage}

\vspace{0.3cm}

% Row 2
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/Hadoop_log_distribution.pdf}
\\(d) Hadoop
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/HealthApp_log_distribution.pdf}
\\(e) HealthApp
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/Linux_log_distribution.pdf}
\\(f) Linux
\end{minipage}

\caption{Distribution of log messages across log groups in Loghub-2.0.}
\label{fig:distribution}

\end{figure*}

 %\noindent\textbf{\textit{}}

==> sections/Motivation.tex <==
\section{Motivation}
\anran{Flow work-in-progress:}
 \begin{figure}[!t]
    \centering
     \includegraphics[width=0.99\columnwidth]{figures/Log_distrubution.png}
    \caption{Distribution of log groups over bench marks.}
     \label{fig:longtail1}
 \end{figure}
 \noindent\textbf{\textit{}}
System logs play a key role in understanding system behavior. They record runtime activity, configuration changes, failures, and abnormal events, which makes them essential for debugging ~\cite{xu2009detecting,Yuan2010Sherlog,chen2019empirical,chen2021pathidea}, monitoring ~\cite{Wang2021QuickPeek,Chen2019LoadTests}, anomaly detection~\cite{Chen2019LoadTests,he2017towards,Su2024LLMForecasting,LibreLog2024}, and root-cause analysis. Syntax-based parsers such as Drain and Spell rely on heuristic rules, frequent pattern mining, or tree-based methods. These approaches are efficient and work well for common log patterns, but their performance drops sharply when they encounter rare logs or logs with irregular formatting.

Real systems naturally follow a long-tail distribution: a small number of log templates produce most of the messages, while many other templates appear only a few times \cite{DivLog2024}. For example, in the Thunderbird dataset, the top nine log groups account for more than 50\% of all logs, while the remaining 1,233 groups occur only a handful of times. Because only a few groups dominate the dataset, most parsers end up learning the frequent patterns and paying very little attention to the rare ones. This is a real problem because rare logs often contain important or unexpected system events. Failing to parse them correctly means missing useful information about what went wrong.

Although some prior work \cite{DivLog2024} discusses the long-tail distribution in SE data and its effect on learning-based methods, its impact on log parsing itself is still not well explored. To highlight this issue, Table~\ref{tab:Table2} shows the performance of a state-of-the-art LLM-based parser, LibreLog \cite{LibreLog2024}, on the Thunderbird dataset. LibreLog reaches 69\% PA on frequent logs, but its accuracy drops sharply to 43\% on infrequent logs. The overall PA still appears to be 69\% only because it is dominated by the large number of frequent logs. This long-tail effect hides the model’s poor performance on rare but important templates. More importantly, although rare logs make up less than 0.01\% of all log entries, their templates represent nearly 25\% of all log groups.
 This significant contrast demonstrates the severity of long-tail challenges in log parsing and underscores the need for a deeper exploration of this issue.
One promising direction is to use Retrieval-Augmented Generation (RAG) together with augmented logs, so we can increase the presence of rare logs inside their rare groups. By retrieving similar or augmented examples before generation, the model receives more helpful context and becomes better at understanding and parsing these low-frequency patterns.

==> sections/RQ.tex <==
\subsection{Research Questions}
we evaluate \tool using the following research questions(RQs):

\begin{itemize}
    \item\textbf{RQ1: How effective is \tool on rare logs?}
    \item\textbf{RQ2: How do different settings affect \tool?}
    \item\textbf{RQ3: Does the proposed augmentation component improve rare log parsing across different LLM-based parsers?}
    \item\textbf{RQ4: How effective is \tool on entire benchmark?}
    
    \item\textbf{RQ5: How efficient is \tool?}
   
\end{itemize}


==> sections/Related_work0.tex <==
\section{Related work}
 %log parsing algorithms can be divided into two main categories: syntax-based~\cite{AEL2008,Drain2017,Logram2020,Spell2019} and semantic-based~\cite{LILAC2024,HighPrecision2024,LLMParser2024,LibreLog2024,DivLog2024}. Syntax-based parser~\cite{AEL2008,Drain2017,Logram2020,Spell2019} refers to those parsers that use heuristic rules, they try to find logs structure through comparison components to identify suitable pattern they mostly focus on how logs look rather than their meaning. for example, AEL~\cite{AEL2008} use huristic methods to eliminate potential dynamic variables and extract log template. Drain~\cite{Drain2017} use fix-depth tree and parsing rules to classify logs and find common templates. However, these methods perform worse when they come up with new logs with undefined rules. Spell~\cite{Spell2019} uses longest common subsequence to parse logs. Logram~\cite{Logram2020} identify frequent n-gram pattern within logs, subsequently it uses these repetitive patterns to parse logs. However, these methods perform poorly when they face new log formats that don’t follow predefined rules, their parsing accuracy completely depends on structure of input logs so, complex structure leads to poor pattern and consequently low accuracy. In short, syntax-based parsers are simple and efficient for common patterns, but their performance varies depending on log structure. In contrast, semantic-based~\cite{LILAC2024,HighPrecision2024,LLMParser2024,LibreLog2024,DivLog2024}parsers try to recognize pattern base on the meaning of context. They look at logs like normal sentence and focus on meaning of it rather than structure. These parsers use machine learning (ML) algorithms, natural language processing (NlP) and language models to identify which part is static or dynamic. In appreciate of LLMS like GP-3, GPT5 or Llama~\cite{Llama3_2024} semantic parser are more likely to become stronger and shown superior accuracy compare to syntax-based ones. Several studies demonstrate these improvements. For instance, DivLog~\cite{DivLog2024} use GPT-3 to select similar logs samples for in-context learning (ICL) to help understanding structure of logs precisely. LILAC~\cite{LILAC2024} use ChatGPT and cashing system so it does not need to do extra parsing time for same logs which consequently leads to saving time and cost. However, both DivLog~\cite{DivLog2024} and LILAC~\cite{LILAC2024} as they use commercial version of LLMS there is risk of data leakage and privacy, especially if logs include sensitive data. To reduce this risk many researchers decided to use open-source version of LLMS like Llama~\cite{Llama3_2024}. Hooglle~\cite{HighPrecision2024} fine-tuned small open-source LLMS with labeled logs. LogPPT~\cite{LogPPT2023} uses masked-language model (RoBerTa~\cite{RoBERTa2019}) to distinguish static and dynamic parts. LLMparser~\cite{LLMParser2024} test various open-source LLMS with few-shot learning. These approaches outperform syntax-based parsers, but they still require preparing example pairs (log–template), which is time-consuming. LibreLog~\cite{LibreLog2024} use combination of cash memory, open-source LLMS, few-shot prompting, and self-reflection steps to achieve high parsing accuracy, lower cost, and better privacy protection while also improving self-correction. Although the results of recent approaches are promising, having deeper insight to their methods show that all focus on improving PA and GA without considering the importance of rare logs, rare log groups, and imbalanced distribution of logs among groups. Such issues can directly affect the quality of parsing and ICL sampling. In this paper, we propose \tool, a new log parser that focuses on rare log events and address this problem through data augmentation to achieve more stable and fair log parsing performance.
 
%Log parsing approaches can be broadly categorized into two main themes: syntax-based methods and semantic-based methods.

%\phead{Syntax-based methods.} Traditional log parsers rely on heuristic rules and structural templates to extract templates~\cite{AEL2008,Drain2017,Logram2020,Spell2019}. These methods focus on how logs look rather than their meaning. For example, AEL~\cite{AEL2008} removes dynamic variables using heuristic rules, while Drain~\cite{Drain2017} organizes logs using a fixed-depth tree. Other approaches such as Spell~\cite{Spell2019} and Logram~\cite{Logram2020} identify templates using longest common subsequence and n-gram frequency, respectively. These methods are efficient and perform well on frequent and well-structured logs. However, their performance degrades when logs contain new formats or complex structures, since they depend heavily on predefined rules.

%\phead{Semantic-based methods.} Recent work uses machine learning and language models to capture the meaning of log messages~\cite{LILAC2024,HighPrecision2024,LLMParser2024,LibreLog2024,DivLog2024,wang2026small,zhang2025logbase}. These approaches treat logs as natural language and aim to identify static and dynamic parts based on context. With the development of LLMs such as GPT~\cite{chatgpt2026} and LLaMA~\cite{Llama3_2024}, semantic-based parsers achieve higher accuracy than syntax-based methods. For instance, DivLog~\cite{DivLog2024} uses GPT-3~\cite{GPT3_2020} for in-context learning, and LILAC~\cite{LILAC2024} uses caching to improve efficiency. Other approaches rely on open-source models to address privacy concerns. Hooglle~\cite{HighPrecision2024} fine-tunes small models, LogPPT~\cite{LogPPT2023} uses masked language models, and LLMParser~\cite{LLMParser2024} applies few-shot learning. LibreLog~\cite{LibreLog2024} further improves performance by combining open-source LLMs with memory and iterative validation.

%\phead{Limitations and research gap.} Although semantic-based methods improve parsing accuracy, they still have several limitations. Many approaches require labeled examples or carefully designed prompts, which increases cost and effort. In addition, most existing methods focus on improving overall metrics such as PA and GA, without considering the impact of data imbalance. In real-world logs, distributions are highly skewed, with many rare log groups. These rare events are often critical for system diagnosis, yet they are underrepresented and difficult to parse.

%\phead{Our approach.} To address this gap, we propose \tool, a log parsing framework that explicitly focuses on rare log events. Instead of only optimizing overall accuracy, \tool improves robustness under long-tailed distributions by using semantic recognition and data augmentation. This allows the model to generate more balanced training signals and achieve more stable and fair performance across both frequent and rare log groups.

We categorize existing log parsers into two broad families: syntax-based and semantic-based methods.

\phead{Syntax-based parsers.} 
Traditional log parsers rely on heuristic rules and structural patterns to extract log templates~\cite{AEL2008,Drain2017,Logram2020,Spell2019}. For example, AEL~\cite{AEL2008} removes dynamic variables using heuristic rules, Drain~\cite{Drain2017} organizes logs using a fixed-depth parsing tree, Spell~\cite{Spell2019} applies longest common subsequence matching, and Logram~\cite{Logram2020} identifies frequent \textit{n}-gram patterns. These methods are efficient and effective for logs with recurring structural patterns. However, because they rely primarily on syntactic similarity, they often struggle to generalize to unseen log formats and complex log structures.
% Traditional parsers rely on heuristic rules and structural patterns to extract log templates~\cite{AEL2008,Drain2017,Logram2020,Spell2019}. Examples include AEL~\cite{AEL2008}, which removes dynamic variables using heuristic rules, Drain~\cite{Drain2017}, which organizes logs using a fixed-depth tree, Spell~\cite{Spell2019}, which applies longest common subsequence matching, and Logram~\cite{Logram2020}, which identifies frequent n-gram patterns. These methods are efficient and perform well on frequent and well-structured logs, but their performance often degrades when logs contain unseen formats or complex structures.

\phead{Semantic-based parsers.} Recent approaches leverage machine learning and language models to capture the semantic meaning of log messages~\cite{LILAC2024,HighPrecision2024,LLMParser2024,LibreLog2024,DivLog2024,wang2026small,zhang2025logbase}. With the emergence of LLMs such as GPT~\cite{chatgpt2026} and Llama~\cite{Llama3_2024}, these methods generally achieve higher parsing accuracy than syntax-based approaches. 
For example, DivLog~\cite{DivLog2024} and LLMParser~\cite{LLMParser2024} leverage in-context learning to improve template inference. LILAC~\cite{LILAC2024} further improves efficiency through cache-based optimization, while LogPPT~\cite{LogPPT2023} employs a masked language model with few-shot learning to classify log tokens. LibreLog~\cite{LibreLog2024} advances this direction by combining LLMs with memory and iterative validation. More recently, EFParser~\cite{wang2026small} further enhances parsing through adaptive cache management and template validation.
However, these approaches still struggle to accurately recover templates for rare log groups because limited structural evidence makes it difficult to distinguish template tokens from variables. To address this gap, we propose \tool, a log parsing framework that enriches rare log groups with representative synthetic log instances before template inference. This design increases the structural evidence available for template recovery while preserving the original log semantics and template structure.

% For example, DivLog~\cite{DivLog2024} and LLMParser~\cite{LLMParser2024} leverage in-context learning, LILAC~\cite{LILAC2024} improves efficiency through cache-based optimization, Hooglle~\cite{HighPrecision2024} fine-tunes small open-source models, LogPPT~\cite{LogPPT2023} uses masked language models, and LibreLog~\cite{LibreLog2024} combines open-source LLMs with memory and iterative validation.

% \phead{Limitations and research gap.} Although semantic-based methods improve parsing accuracy, most focus primarily on overall metrics such as PA and GA. In practice, log distributions are highly imbalanced, with many rare log groups that are difficult to parse but often important for system diagnosis. Existing work largely overlooks the impact of such long-tailed distributions on parsing performance.

% \phead{Our approach.} To address this gap, we propose \tool, a log parsing framework that explicitly targets rare log events. \tool combines semantic recognition and template-preserving augmentation to strengthen sparse log groups, improving robustness under long-tailed distributions and achieving more stable performance across both frequent and rare logs.


==> sections/data_collection.tex <==
\section{Data Collection}
To address the limitations of existing log-parsing algorithms that overlook infrequent events, our study focuses specifically on rare logs and rare log groups. For this purpose, we created new ground-truth files for each dataset, containing log events with fewer than five instances. We then conducted experiments on these revised datasets to evaluate how well our proposed algorithm performs compared to existing methods.


==> sections/int.tex <==
\section{Introduction}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/Example_Log.png}
    \caption{Example log parsing from the Linux dataset.}
    \label{fig:logexample}
\end{figure}

\anran{@Sepideh, I’ll try to document my thought process when making revisions to the paper using *note* comments. Please make sure to go through them carefully, and fix *fixme* comments}
\anran{Some general feedback: 1) Unify the terms throughout the paper (e.g., log pattern vs. parsed templates vs. structured logs)}

 
\note{Software engineering context, importance of logs}
Software systems continuously generate large volumes of logs during execution. These logs provide a detailed record of system execution, such as runtime events, system states, warnings, and failures. In modern software engineering, collection and examination of such logs, commonly referred to log analysis, which play a critical role in a wide range of activities, including
% System logs are one of the most important sources for understanding system behavior. 
% They record runtime activities, configuration changes, failures, and anomalies, and are widely used for 
software debugging~\cite{xu2009detecting,Yuan2010Sherlog,chen2019empirical,chen2021pathidea}, monitoring~\cite{Wang2021QuickPeek,Chen2019LoadTests,candido2021logbased,razavi2008pattern}, anomaly detection~\cite{Chen2019LoadTests,he2017towards,Su2024LLMForecasting,LibreLog2024,huo2023semparser,Zhang2020UnstableLogs,he2016loganalysis,sun2026improving}, and root cause analysis~\cite{lu2017logbased,zawawy2010log,suriadi2012root,mariani2008automated}. 
As software systems become increasingly complex, developers rely on automated analysis of log to maintain system reliability and availability.

\note{What are log messages, reference to Figure 1, why logs are challenging to analyze (semi-structure), log parsing as a solution}
\anran{The content is good, but you should clearly define and connect the key concepts throughout the introduction. In particular, explain what log messages are, how they are generated, what log analysis is, and where log parsing fits within the log analysis pipeline.}
Log messages are generated by logging statements in the source code. A logging statement consists of a static text template and runtime variables whose values are instantiated during system execution. Hence, log messages are semi-structured in nature: messages generated from the same logging statement share a common template but differ in their variable content. Figure~\ref{fig:logexample} illustrates an example of log messages from the Linux dataset. The first two messages are generated from the same logging statement and therefore share a common log template.Specifically, they contain identical static text while differing only in their dynamic parameter values.However, third line come from other log statement with different template.  
\fixme{explain that the first two raw messages share the same template, explain static vs. dynamic}. While this structure makes logs easy to read for developers, the presence of dynamic variables makes automated log analysis challenging. To enable downstream log analytics tasks, including anomaly detection~\cite{Chen2019LoadTests,he2017towards,Su2024LLMForecasting,LibreLog2024,huo2023semparser,Zhang2020UnstableLogs,he2016loganalysis,sun2026improving}, failure prediction~\cite{das2020failure,lim2008log,zheng2009system,zhang2016automated}, and root cause analysis~\cite{lu2017logbased,zawawy2010log,suriadi2012root,mariani2008automated}, raw log messages must first be transformed into structured template through log parsing.
% However, raw logs are typically semi-structured or unstructured, making them difficult to analyze directly. Log parsing addresses this challenge by transforming raw log messages into structured templates, separating constant text from dynamic variables as illustrated in Figure~\ref{fig:logexample}. Accurate log parsing is therefore a fundamental step for reliable downstream log analysis.

\note{Traditional log parsers, LLM-based log parsers, despite their effectiveness, they rely on sufficient examples to infer template structure.}
Traditional log parsers, such as Drain~\cite{Drain2017} and Spell~\cite{Spell2019}, rely on heuristic rules or tree-based structures to extract templates. These approaches are efficient and perform well when log templates are repetitive and consistent.
More recently, large language model (LLM)-based log parsers have been proposed to improve parsing accuracy by leveraging semantic understanding of log messages\fixme{cite}. Compared to rule-based approaches, these methods are more flexible and can better handle diverse log formats.

\input{figures/Motivation_example}
In practice, log data are often highly imbalanced, where a small number of log templates account for the majority of log messages while many templates appear only a few times. This phenomenon arises naturally because common system behaviors repeatedly generate the same log templates, whereas failures, exceptional events, and uncommon execution paths occur rarely~\cite{}\fixme{}. As a result, some templates provide abundant evidence for template inference, while others are represented by only a handful of log messages. Recent work by Jiang et al.~\cite{jiang2024large} demonstrated that parser performance varies across template frequencies, and that templates that appear less frequently remain difficult to parse. Table~\ref{tab:example} illustrates a motivating example from the Mac dataset. While LibreLog~\cite{LibreLog2024}, a state-of-the-art LLM-based log parser, achieves 100\% parsing accuracy on the frequent template ``E113'', which accounts for 7.7\% of all log messages. In contrast, its accuracy drops to 0\% on the rare template ``E164'', which appears only three times. These observations suggest that limited structural evidence may substantially affect template inference for underrepresented log groups.

However, it remains unclear how prevalent such rare log groups are in real-world systems, whether existing evaluation metrics adequately reflect their impact on parser robustness, and how parsing performance can be improved under highly imbalanced log distributions.
% \anran{@continue here}
% \note{In production systems, logs are often imbalanced ... small number of log templates account for the majority of log messages ... existing studies report accuracy without explicitly examining how parsers perform on rare log templates (define rare log templates) ... masking poor performance on underrepresented templates ...}
% \note{Examining this data imbalance is crucial ... robustness of existing log parser may be affected. Table~\ref{} demonstrates ... To the best of our knowledge, the prevalence of log data imbalance in real-world log datasets and its implications for log parsing performance remain largely unexplored in the literature ... The only related work we found come from Jiang et al. ...}
% \anran{We don't know yet if they follow a long-tailed distribution, use data imbalance instead}
% Despite these advances, existing log parsing methods implicitly assume that sufficient examples are available for each log pattern. However, this assumption does not hold in real-world systems. In practice, log data often follow a long-tailed distribution, where a small number of frequent log patterns dominate the dataset, while a large number of log patterns appear only a few times. These rare log groups often correspond to abnormal executions, failures, or uncommon system behaviors, and are therefore critical for system diagnosis.
% Under long-tailed distributions~\cite{wang2013using,song2018comprehensive,Zhou2023DevilInTheTails}, reliable template inference becomes significantly more difficult. When only a few instances are available for a log pattern, parsers lack sufficient evidence to reliably infer its template structure. As a result, existing methods including both rule-based and LLM-based tend to perform well on frequent logs but struggle significantly on rare ones. For rule-based methods, insufficient repetition makes it difficult to discover stable patterns. For LLM-based methods~\cite{LLMParser2024,LibreLog2024,LILAC2024,DivLog2024}, limited examples increase the risk of incorrect template generation or hallucinated structures. Importantly, this degradation is often hidden in standard evaluations, where overall accuracy is dominated by frequent log patterns and fails to reflect errors on rare but critical groups.
% Recent work by Jiang et al~\cite{jiang2024large}. investigates the impact of log frequency on parsing performance and reports that existing parsers exhibit varying effectiveness when dealing with different occurrence frequencies. 
% However, their analysis primarily provides high-level observations and does not explicitly focus on rare log groups as a distinct challenge under long-tailed distributions. In particular, they do not systematically evaluate how performance degrades on rare logs, nor do they explore methods to improve robustness under data imbalance.
\fixme{1) Large-scale empirical study: rare logs are common at the template level. 2) Evaluation on the state-of-the-art: existing parsers degrade substantially on rare logs. 3) Our study reveals that commonly used evaluation metrics may overestimate parser robustness because frequent log groups dominate overall performance measurements.}

\fixme{3) Motivated by these findings, we propose TRAIL: improves robustness under imblanced log distributions by augmenting rare log groups before template inference. 4) TRAIL improve rare-log parsing accuracy by up to 19.4\%\anran{to verify} compared to the strongest state-of-the-art while maintaining competitive performance on complete datasets.}
% To address this challenge, we first conduct a large-scale empirical study on the LogHub-2.0 benchmark to analyze the prevalence and impact of rare log groups. Our study shows that rare logs constitute nearly 20\% of all templates but account for less than 0.01\% of log messages, and that all state-of-the-art parsers exhibit significant performance degradation on these logs.We further show that commonly used grouping-based metrics may overestimate parser robustness because frequent log groups dominate the evaluation.Based on these insights, we propose TRAIL\fixme{what does TRAIL stand for?}, an augmentation-driven log parsing framework designed to improve robustness under long-tailed distributions. Instead of directly parsing rare log groups, TRAIL strengthens them before template inference through semantic template generation, structure-preserving augmentation, and diversity-guided sampling. This design provides richer structural evidence for template inference, enabling more accurate parsing even when only a few log instances are available.
% We evaluate TRAIL on the LogHub-2.0 benchmark and compare it with state-of-the-art log parsers. The results show that TRAIL significantly improves parsing accuracy on rare log groups while maintaining competitive performance on full datasets. These findings highlight the importance of rare-log-aware evaluation and demonstrate that addressing data imbalance is essential for reliable log parsing in real-world systems.

%System logs are one of the most important sources for understanding system behavior. They record runtime activities, configuration events, failures, and anomalies. Because of this, they are widely used for debugging~\cite{chen2019empirical,chen2021pathidea}, monitoring ~\cite{Wang2021QuickPeek,Chen2019LoadTests}, anomaly detection ~\cite{Chen2019LoadTests,he2017towards,Su2024LLMForecasting,LibreLog2024,huo2023semparser,Zhang2020UnstableLogs,he2016loganalysis}, and root cause analysis~\cite{lu2017logbased}.
%However, raw logs are usually semi-structured or unstructured text. This makes analysis difficult. Log parsing is the process of extracting structured templates from raw log messages by separating constant and variable parts, as illustrated in Figure~\ref{fig:logexample}. 

%As a result, many downstream log analysis tasks rely on accurate log parsing.


%Traditional log parsers, such as Drain ~\cite{Drain2017} and Spell ~\cite{Spell2019}, use heuristic rules or tree-based machine learning methods. These approaches are efficient and work well for common log patterns. Recently, LLM-based log parsers have been proposed as a promising alternative to traditional methods~\cite{LLMParser2024,LibreLog2024,LILAC2024,DivLog2024}. Instead of relying on fixed rules or heuristics, these approaches leverage semantic understanding to identify patterns in log messages. As a result, they often achieve better performance, especially when handling complex or diverse log formats.
%\anran{Talking about rare logs here is premature, we haven't justified it is an issue yet}
%\anran{Another problem, listing too many issues in LLMs weakens the focus, our motivation is about data distribution}
%However, LLM-based parsers also have several limitations. They may produce incorrect templates due to hallucination~\cite{zhang2025hallucinations,Le2023ChatGPTLogParsing}, 
%and their performance often depends heavily on the quality and coverage of the input examples, which can be difficult to ensure in practice~\cite{LibreLog2024,Jiang2024}.
%In practice, this makes them sensitive to the distribution of log data.


%\anran{check}
%A key challenge in real-world log parsing is data imbalance, which often follows a long-tailed distribution. In practice, log datasets typically contain a small number of frequent patterns and a large number of rare ones, a phenomenon commonly observed in software engineering data~\cite{wang2013using,song2018comprehensive,Zhou2023DevilInTheTails}. Such imbalance makes template inference more difficult and may reduce parser robustness when handling rare logs. Recent work by Jiang et al.~\cite{jiang2024large} is among the first to investigate the impact of log frequency on parsing performance, showing that parser accuracy can vary across logs with different occurrence frequencies. However, there is still no systematic study on how long-tailed log distributions affect log parsing as a whole, and existing parsers do not explicitly account for rare log groups, even though such events are often critical for system diagnosis.

%\anran{check, avoid selling on the approach}
%To address these challenges, we first conduct an empirical study to understand how long-tailed distributions affect log parsing. We characterize rare log groups and define them as templates with fewer than five instances, which allows us to systematically analyze their prevalence and impact. Our study on LogHub-2.0 shows that a strong long-tail distribution, where a few log groups generate most messages while many rare groups
%occur only a few times but may correspond to critical system events. Furthermore, we observe that existing log parsing methods perform well on frequent
%log patterns but struggle significantly with rare logs. 

%Based on these observations, we design TRAIL, a log parsing framework intended to improve robustness under long-tailed distributions. Rather than changing the overall parsing pipeline, TRAIL strengthens rare log groups before template inference through semantic template generation, log augmentation, and diversity sampling. These steps aim to provide more reliable evidence for template generation when only a few log instances are available. Our experimental results show that this design leads to more balanced performance across both frequent and rare logs, while maintaining competitive accuracy on full datasets.

In short, this paper makes the following key contributions:
\begin{itemize}[leftmargin=*]
    \item To the best of our knowledge, we are the first to study the prevalence of rare logs and its impact on log parsing. We show that existing log parsing evaluations can overestimate parser robustness by masking performance degradation on rare log groups.
    \item We introduce TRAIL, an augmentation-driven framework designed to improve the robustness of state-of-the-art log parsers under imbalanced log distributions.
    \item We demonstrate the generalizability of our augmentation strategy by improving state-of-the-art LLM-based parsers while preserving their original designs.
    % \item We present the one of the first large-scale empirical study on the impact of long-tailed log distributions on log parsing. Across 13 datasets containing over 50 million log messages, we show that real-world logs exhibit severe imbalance, which significantly affects the robustness of existing parsers.
    % \item We re-evaluate five state-of-the-art log parsers under long-tailed settings and show that their performance degrades substantially on rare log groups.
    % \item We propose TRAIL, a rare-group enhancement log parsing framework designed for long-tailed log distributions. It strengthens rare log groups through semantic template generation, log augmentation, and diversity sampling to enable reliable template inference under highly imbalanced data.
    \item To facilitate future research, we make our replication package publicly available at \url{https://anonymous.4open.science/r/TRAIL-B590/}.
\end{itemize}


% The rest of this paper is organized as follows. Section~2 presents the empirical study on rare logs. Section~3 presents our proposed approach. Section~4 presents our study design. Section~5 describes the experimental setup and results. Section~6 presents threats to validity. Section~7 reviews related work. Section~8 presents the discussion. Finally, Section~9 concludes the paper.



\begin{figure*}[t]
\centering

% Row 1
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{figures/Thunderbird_log_distribution.png}
\\(a) Thunderbird
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{figures/Mac_log_distribution.png}
\\(b) Mac
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{figures/BGL_log_distribution.png}
\\(c) BGL
\end{minipage}

\vspace{0.3cm}

% Row 2
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{figures/Hadoop_log_distribution.png}
\\(d) Hadoop
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth, keepaspectratio]{figures/HealthApp_log_distribution.png}
\\(e) HealthApp
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth,keepaspectratio]{figures/Linux_log_distribution.png}
\\(f) Linux
\end{minipage}

\caption{Distribution of log messages across log groups in Loghub-2.0.}
\label{fig:distribution}

\end{figure*}

 \noindent\textbf{\textit{}}

==> setup.tex <==
% \usepackage{cite}
% \usepackage[hidelinks]{hyperref}
% \usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage[dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{xspace}
\usepackage{enumitem}

\usepackage[most]{tcolorbox}
\tcbset{
  leftlineonly/.style={
    enhanced,
    breakable,
    colback=gray!8,  
    boxrule=0pt,             
    colframe=white,           
    arc=8pt,                  
    left=6pt, right=4pt, top=4pt, bottom=4pt
  }
}

\newcommand{\gain}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\drop}[1]{\textcolor{red}{#1}}

% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


\newcommand{\anran}[1]{\textcolor{red}{{\it [AnRan says: #1]}}}
\newcommand{\fixme}[1]{\textcolor{orange}{{\it [fixme #1]}}}
\newcommand{\xinyu}[1]{\textcolor{blue}{{\it [Xinyu says: #1]}}}
\newcommand{\zhenhao}[1]{\textcolor{blue}{{\it [Zhenhao: #1]}}}
\newcommand{\sepideh}[1]{\textcolor{purple}{{\it [sepideh says: #1]}}}
\newcommand{\note}[1]{\textcolor{orange}{{\it [Note: #1]}}}


\newcommand{\rqboxc}[2]{%
  \begin{tcolorbox}[
    enhanced,
    colback=white,
    colframe=black,
    coltitle=white,
    fonttitle=\bfseries,
    title=#1,
    attach boxed title to top left,
    boxed title style={
      colframe=black,
      colback=black,
      size=small,       
      sharp corners=south
    },
    sharp corners,
    boxrule=1pt,
    left=4pt, right=4pt, top=4pt, bottom=4pt
  ]
  #2
  \end{tcolorbox}%
}

\newcommand{\rqboxnew}[2]{%
  \begin{tcolorbox}[
    enhanced,
    title=#1,
    boxrule=1pt,
    left=4pt, right=4pt, top=4pt, bottom=4pt
  ]
  #2
  \end{tcolorbox}%
}


% new paragraph without indent, bold
\newcommand{\phead}[1]{\vspace{1mm} \noindent {\bf #1}}
% new paragraph without indent, underlined
\newcommand{\uhead}[1]{\noindent {\underline {#1}}}
% new paragraph without indent, italic
\newcommand{\ihead}[1]{\noindent {\textit {#1}}}
% new paragraph without indent, italic, underlined
\newcommand{\iuhead}[1]{\noindent {\ul {\textit {#1}}}}
% inline code style 1
\newcommand{\inlinecode}{\texttt}
% inline code style 2
\newcommand{\inlineCode}{\lstinline[basicstyle=\normalsize\ttfamily]}


\newcommand{\tool}{TRAIL\xspace}

% \usepackage{listings}

% \lstset{
%   basicstyle=\ttfamily\footnotesize, 
%   breaklines=true,                   
%   frame=lines,                       
%   postbreak=\mbox{\textcolor{gray}{$\hookrightarrow$}\,},
% }



\begin{comment}
\newcommand{\rqboxc}[2]{%
  \begin{tcolorbox}[
    enhanced,
    colback=white,
    colframe=black,
    coltitle=white,
    fonttitle=\bfseries,
    title=#1,
    attach boxed title to top left,
    boxed title style={
      colframe=black,
      colback=black,
      size=small,       
      sharp corners=south
    },
    sharp corners,
    boxrule=1pt,
    left=4pt, right=4pt, top=4pt, bottom=4pt
  ]
  #2
  \end{tcolorbox}%
}
\end{comment}
